Adaptive Finite Element Methods

This is a survey on the theory of adaptive finite element methods (AFEMs), which are fundamental in modern computational science and engineering but whose mathematical assessment is a formidable challenge. We present a self-contained and up-to-date discussion of AFEMs for linear second order elliptic PDEs and dimension d>1, with emphasis on foundational issues. After a brief review of functional analysis and basic finite element theory, including piecewise polynomial approximation in graded meshes, we present the core material for coercive problems. We start with a novel a posteriori error analysis applicable to rough data, which delivers estimators fully equivalent to the solution error. They are used in the design and study of three AFEMs depending on the structure of data. We prove linear convergence of these algorithms and rate-optimality provided the solution and data belong to suitable approximation classes. We also address the relation between approximation and regularity classes. We finally extend this theory to discontinuous Galerkin methods as prototypes of non-conforming AFEMs and beyond coercive problems to inf-sup stable AFEMs.

==> convergence-bk.tex <==

Our intent in this section
is to design and analyze a {\it two-step AFEM} for the model problem \eqref{strong-form},
as first proposed by R. Stevenson \cite{Stevenson:08}, and further explored in
\cite{BonitoDeVoreNochetto:2013,CohenDeVoreNochetto:2012}. This allows us to
approximate a load term $f\in H^{-1}(\Omega)$ and discontinuous coefficients
$\bA$ and $c$ within the same framework. We will extend this approach to the
Stokes system, and related
saddle point problems, in Section \ref{S:conv-rates-infsup}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\bf Structure of AFEM}\label{S:structure-AFEM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The idea is to concatenate the modules $\DATA$ and $\GALERKIN$ as follows:
given an initial mesh $\mesh_0$ and parameters $\varepsilon_0>0$, $0<\omega\le1$,
$\AFEM$ sets $k=0$ and iterates \looseness=-1
%
\medskip
%
\begin{algotab}
  \>  $[\widehat\mesh_{k},\widehat\data_{k}]= \DATA \, (\mesh_k, \data, \omega \, \varepsilon_k)$ \\
  \>  $[\mesh_{k+1},u_{k+1}]= \GALERKIN \, (\widehat{\mesh}_{k},\widehat\data_{k},\varepsilon_k)$ \\
  \>  $\varepsilon_{k+1}=\tfrac12 {\varepsilon_k}; ~ k \leftarrow k+1$
\end{algotab}
%
\medskip\noindent
%
Let's discuss the two modules for one single iteration
and drop the subscript $k$ for notational convenience.
We recall that data $\data = (\bA,c,f)$ satisfies
%
\begin{equation}\label{E:space-data}
\data \in \X := L^\infty(\Omega; \R^{d\times d})  \times L^\infty(\Omega) \times H^{-1}(\Omega).
\end{equation}
%
The module $\DATA$, discussed in Section \ref{S:data-approx}, approximates $\data$
by discrete data
%
\begin{equation}\label{E:space-discrete-data}
  \widehat\data = (\wh\bA, \wh{c}, \wh{f}) \in \X_{\wh\grid} := \big[ {\mathbb S}^{n-1,-1}_{\wh{\grid}} \big]^{d\times d}
\times {\mathbb S}^{n-1,-1}_{\wh{\grid}} \times \disfct_{\wh{\grid}}
\end{equation}
%
subordinate to an admissible refinement $\widehat\mesh$ of $\mesh\in\grids$
to accuracy $\omega \, \varepsilon$ within the product space
%
\begin{equation}\label{E:approx-space}
  D(\Omega) := L^\infty(\Omega; \R^{d\times d}) \times W^{-s}_q(\wh\grid) \times H^{-1}(\Omega).
\end{equation}
%
Here $2\le q \le \infty$ and $s>0$ are suitable exponents, and
$W^{-s}_q(\wh\grid)=\Pi_{T\in\wh\grid}W^{-s}_q(T)$ stands for the broken space over
$\wh\grid\in\grids$. We recall that $\wh{f}=P_{\wh\grid} f$ is given by
%
\begin{equation}\label{E:discrete-load}
\wh{f} = \sum_{T\in\wh\grid} q_T \chi_T + \sum_{F\in\wh\faces} q_F \delta_F,
\end{equation}
%
where $\chi_T$ is the characteristic function of $T\in\wh\grid$ and $\delta_F$ is the Dirac mass
supported on $F\in\wh\faces$, the internal faces of $\wh\grid$,
according to \eqref{disfct}.
%
The coefficients $(\bA,c)$ satisfy the following structural assumptions $\bA \in M(\alpha_1,\alpha_2)$
and $c \in R(c_1,c_2)$, where
%
\begin{equation*}\label{E:structural-assumption}
M(\alpha_1,\alpha_2) := \big\{\bA\in L^\infty(\Omega; \R^{d\times d}_{\textrm{sym}}):
\alpha_1\le\lambda_j(\bA(x))\le \alpha_2 \quad\forall x\in\Omega, 1\le j \le d \big\}
\end{equation*}
%
and
\begin{equation*}
R(c_1,c_2) := \big\{ c \in L^\infty(\Omega): c_1 \le c(x) \le c_2 \quad\forall x\in\Omega \big\},
\end{equation*}
%
$\alpha_1 > 0$, $c_1\ge0$ and $\lambda_j(\bA(x))$ denotes the $j$-th eigenvalue of $\bA$ at
$x\in\Omega$; see \eqref{uniform_spd}.
Section \ref{S:data-approx} addresses the important questions of maintaining the positive
definite structure of $\bA$ and the sign condition of $c$, namely
%
\begin{equation}\label{E:structural-assumption}
\wh\bA \in M(\wh\alpha_1,\wh\alpha_2),
\quad
\wh{c} \in R(\wh{c}_1,\wh{c}_2)
\end{equation}
%
with
%
\begin{equation}\label{E:wh-alpha}
\wh\alpha_1 = \wh\alpha_1(\alpha_1,\alpha_2) \ge \frac{\alpha_1}{2},
\quad
\wh{c}_1= \wh{c}_1(c_1,c_2,\alpha_1) \ge -\frac{\alpha_1}{4C_P^2},
\end{equation}
%
where $C_P>0$ is the Poincar\'e constant in \eqref{E:Poincare}.
This implies coercivity and continuity of the perturbed bilinear form $\wh\B$
%
\begin{equation*}
\wh\B[\hu,v] := \int_\Omega \nabla v \cdot \wh\bA \nabla\hu + \wh{c} v\hu
\end{equation*}
%
because for all $v,w \in H^1_0(\Omega)$
%
\[
\wh\B[v,v] \ge \int_\Omega \halpha_1 |\nabla v|^2 - \wh{c}_1 |v|^2
\ge \big(\halpha_1- \wh{c}_1 C_P^2\big) \int_\Omega |\nabla v|^2
\ge \frac{\alpha_1}{4} |v|_{H^1_0(\Omega)}^2
\]
%
and
%
\[
\big|\wh\B[v,w] \big| \le \int_\Omega \halpha_2 |\nabla v| \, |\nabla w + \wh{c}_2 |v| \, |w|
\le \big(\halpha_2 + \wh{c}_2 C_P^2) |v|_{H^1_0(\Omega)} |w|_{H^1_0(\Omega)}
\]
%
Therefore, the energy norm $\enorm{v}^2 = \wh\B[v,v]$ is equivalent to the $H^1_0$-seminorm
%
\begin{equation}\label{E:enorm-Vnorm-wh}
c_{\wh\B} |v|_{H^1_0(\Omega)}^2 \le \enorm{v}^2 \le C_{\wh\B} |v|_{H^1_0(\Omega)}^2,
\end{equation}
%
and the constants $0<c_{\wh\B} \le C_{\wh\B}$ are explicitly related to
$0<c_{\B} \le C_{\B}$ in \eqref{nsv-enorm-Vnorm} and are independent of $k$.
The Lax-Milgram Theorem thus guarantees the
existence of a unique solution $\hu\in \V=H^1_0(\Omega)$ of the perturbed problem
%
\begin{equation}\label{E:perturbed-pb}
    \hu\in \V:\quad \wh\B(\hu,v] =
      \langle \hat{f},v \rangle = \sum_{T\in\wh\grid} \int_T q_T v + \sum_{F\in\wh\faces} \int_F q_F v
      \quad\forall v\in\V.
\end{equation}
%
We later show in Section \ref{S:perturbation} the perturbation estimate
%
\begin{equation}\label{E:perturbation-est}
|u-\hu|_{H^1_0(\Omega)} \le C(\data,\Omega) \, \|\data - \wh\data\|_{D(\Omega)},
\end{equation}
%
and in Section \ref{S:data-approx} prove the error estimate in $D(\Omega)$ for $\data$
%
\begin{equation}\label{E:error-data}
\|\data - \wh\data\|_{D(\Omega)} \le \omega \eps.
\end{equation}
%

The pair $(\widehat{\mesh},\widehat\data)$
is next taken by $\GALERKIN$ to run an inner loop of the form
%
\begin{equation}\label{E:adaptive-loop}
\SOLVE \,\,
\longrightarrow \,\,
\ESTIMATE \,\,
\longrightarrow \,\,
\MARK \,\,
\longrightarrow \,\,
\REFINE
\end{equation}
%
with fixed discrete data $\widehat\data$ and initial mesh
$\widehat{\mesh}$. The module $\GALERKIN$ stops as soon as the error
tolerance $\varepsilon$
is reached, which takes a finite number of iterations because $\GALERKIN$
is a contraction between
consecutive iterates, and creates the next mesh-solution pair $(\mesh,\uG)$.
It is worth noticing that, in the absence of
this stopping test, the Galerkin solution $\uG$ would converge to the solution $\hu\in H^1_0(\Omega)$ of \eqref{E:perturbed-pb}, which is not the desired solution $u$ of
\eqref{strong-form}.

We stress that, in view of \eqref{E:perturbation-est} and \eqref{E:error-data},
the relative resolution of the modules $\DATA$ and $\GALERKIN$ is critical for the discrepancy between
the exact and perturbed solutions $u$ and $\hu$. This is ultimately
responsible for the performance of $\AFEM$ and is studied in Section
\ref{S:conv-rates-coercive}.

To organize the discussion about convergence of $\AFEM$ we first assume that data $\data$
is discrete, i.e. $\data=\hat\data$, the module $\DATA$ is skipped and $\AFEM$ reduces to
$\GALERKIN$. We present this convergence setting in Section \ref{S:discrete-data}, which
is simplified with respect to the standard literature in that we avoid the so called
data oscillation. We tackle in Section \ref{S:general-data} the general case of variable
coefficients, prove \eqref{E:perturbation-est}, and discuss the two-step algorithm $\AFEM$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\bf Convergence for Discrete Data}\label{S:discrete-data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now present the four basic modules of $\GALERKIN$ in \eqref{E:adaptive-loop},
discuss their main properties, and prove a contraction property between
consecutive iterates of $\GALERKIN$. In doing so, we assume that data $\data$ is discrete.

%-------------------------------------------------------------------------------
\subsubsection{\bf Modules of $\GALERKIN$}\label{S:GALERKIN}
%-------------------------------------------------------------------------------

\bigskip\noindent
\textbf{Module $\SOLVE$.}
If $\grid\in\grids$ is a conforming refinement of $\wh\grid$, $\V_\grid$
is the finite element space of $C^0$ piecewise polynomials of degree $\le n$, then 
%
\[
 \uG = \SOLVE \, (\grid)
 \]
 %
determines the Galerkin s       olution \emph{exactly}, namely without algebraic error,
%
\begin{equation}\label{E:galerkin}
  \begin{aligned}
    \uG \in \VG:\quad \B(\uG,v] &= \int_\Omega \nabla v \cdot \bA \nabla\uG + c vu
    = \langle f,v \rangle  \\
      & =
      \sum_{T\in\wh\grid} \int_T q_T v + \sum_{F\in\faces} \int_F q_F v
      \quad\forall v\in\VG.
  \end{aligned}
\end{equation}
%

%-------------------------------------------------------------------------------------
\noindent
\textbf{Module $\ESTIMATE$.} 
Given a conforming mesh $\grid\in\grids$ and the Galerkin solution
$\uG\in\VG$, the output $\{\estG(\uG,T)\}_{T\in\grid}$ of
%
\[
	\{\estG(\uG,T)\}_{T\in\grid}=\ESTIMATE \, (\uG,\grid,\data)
\]
%
are the element indicators defined as follows for any $v\in\V$
%
\begin{equation}\label{E:estimator}
	\estG^2(v,T)=h_T^2\,\|r(v)\|^2_T+h_T\,\|j(v)\|^2_{\partial T}\quad\forall T\in\grid,
\end{equation}
%
where the \emph{interior} and \emph{jump residuals} are given by
%
\begin{equation}\label{E:residuals}
\begin{alignedat}{2}
	& r(v)|_T = q_T+\divo(\bA\nabla v)-cv \quad &&\fa T\in\grid\\
	& j(v)|_F = \big([\bA\nabla v] + q_F \big)\cdot\nu\,|_S \quad &&\fa F\in\faces,
\end{alignedat}
\end{equation}
%
and $j(v)|_F=0$ for boundary faces $F$. We denote
$\estG^2(v,\mathcal{P})= \sum_{T\in\mathcal{P}}\estG^2(v,T)$ for any subset
$\mathcal{P}$ of $\grid$ and
$\estG(v)=\estG(v,\grid)$.
%

%---------------------------------------------------------------------------
\bigskip\noindent  
{\bf Module $\MARK$.}
%---------------------------------------------------------------------------
Given $\grid\in\grids$, the Galerkin solution $\uG\in\V(\grid)$,
and element indicators $\{\estG(\uG,\elm)\}_{\elm\in\grid}$,
the module \MARK selects elements for refinement using
\emph{D\"orfler Marking} (or bulk chasing), \ie given a parameter $\theta\in(0,1]$ 
the output $\marked$ of
%
\begin{displaymath}
  \marked=\MARK\big(\{\estG(\uG,\elm)\}_{\elm\in\grid},\grid\big)
\end{displaymath}
satisfies
\begin{equation}\label{E:theta}
  \estG(\uG,\marked)\ge\theta\,\estG(\uG,\grid).
\end{equation}
%
This marking guarantees that $\marked$ contains a substantial part of
the total (or bulk), thus its name. The choice of $\marked$
does not have to be minimal at this stage, that is, the marked elements
$T\in\marked$ do not necessarily must be those with largest
indicators.

%---------------------------------------------------------------------------
\bigskip\noindent  
{\bf Module $\REFINE$.}
%---------------------------------------------------------------------------
Let $b\in\N$ be the number of desired bisections per marked element.
Given $\grid\in\grids$ and a subset $\marked$ of marked elements, the
output $\gridk[*]\in\grids$ of
%
\begin{displaymath}
  \grid_*=\REFINE\big(\grid,\,\marked\big)
\end{displaymath}
%
is the smallest refinement $\gridk[*]$ of $\grid$ so that
all elements of $\marked$ are at least bisected $b$ times. Therefore,
we have $h_{\grid_*}\leq h_\grid$ and the strict reduction property 
%
\begin{equation}\label{nv-h-reduction}
h_{\grid_*}|_T \leq 2^{-b/d} h_\grid|_T \qquad\fa T\in\marked,
\end{equation}
%
where $h_\grid:\Omega\to\R^+$ is a piecewise constant meshsize function that coincides with
$h_T$ on every $T\in\grid$.
We finally let $\Res=\refined=\grid\backslash\grid_*$ be the subset of refined elements of $\grid$
and note that
%
$
\marked\subset\Res.
$

%------------------------------------------------------------------------------------
\bigskip\noindent
{\bf GALERKIN}: Set $j=0$, let the starting grid be $\grid_0=\wh\grid$, and iterate

\begin{algotab}
  \> $u_j=\SOLVE \, (\grid_j)$;\\
  \> $\{\est_j(u_j,T)\}_{T\in\grid_j} = \ESTIMATE(u_j,\grid_j,\data)$;\\
  \> $\marked_j = \MARK \, \big(\{\est_j(u_j,T)\}_{T\in\grid_j},\grid_j\big)$;\\
  \> $\grid_{j+1} = \REFINE(\grid_j,\marked_j)$; $j\leftarrow j+1$.
\end{algotab}



%-------------------------------------------------------------------------------
\subsubsection{\bf Basic properties of $\GALERKIN$}\label{S:basic-properties}
%-------------------------------------------------------------------------------

We next follow Casc\'on, Kreuzer, Nochetto, and Siebert
\cite{CaKrNoSi:08} and summarize some basic properties of AFEM that
emanate from the symmetry of the differential operator (i.e. of $\bA$ and $c$)
and features of the modules. In doing this, any explicit constant or hidden constant
in $\Cleq$ will only
depend on the uniform shape-regularity of $\grids$, the dimension $d$,
the polynomial degree $n$, and the (global) eigenvalues of $\bA$, but
not on a specific grid $\grid\in\grids$, except if explicitly stated. 
Furthermore, $u$ will always
be the weak solution of \eqref{E:perturbed-pb}.

The following property relies on the fact that the perturbed bilinear
form $\B$ is coercive and
symmetric, and so induces a scalar product in $\V$ equivalent to the
$H^1_0$-scalar product; see \eqref{E:enorm-Vnorm-wh}.
%
\begin{lemma}[Pythagoras]\label{L:Pythagoras}
  Let $\grid_*\in\grids$ be a conforming refinement of $\grid\in\grids$. The
  corresponding Galerkin solutions $\uG\in\V_\grid$ and
  $u_{\grid_*}\in\V_{\grid_*}$ satisfy the orthogonality property
%
\begin{equation}\label{E:Pythagoras}
	\enorm{u-\uG}^2=\enorm{u-u_{\grid_*}}^2+\enorm{u_{\grid_*}-\uG}^2.
\end{equation}  
\end{lemma}
%
\begin{proof}
Exploit that $\B$ is a scalar product and $\B[u-u_{\grid_*},u_\grid,u_{\grid_*}]=0$.
\end{proof}

Property \eqref{E:Pythagoras} is valid for \eqref{strong-form} for the energy
norm exclusively. This restricts the subsequent analysis to the
energy norm, or equivalent norms, but does not extend to other,
perhaps more practical, norms such as the maximum norm. This is an
important open problem and a serious limitation of this theory.

\begin{proposition}[a posteriori error estimates]\label{L:ApostEnergy}
  There exist constants $0<C_2\le C_1$, depending on the shape regularity of $\grids$ and
  $c_\B\le C_\B$ in \eqref{nsv-enorm-Vnorm}, such that for any
  $\grid\in\grids$ and the corresponding Galerkin solution
  $\uG\in\VG$ there holds
%
  \begin{equation}\label{E:aposteriori-bounds}
    C_2\,\estG(\uG) \le \enorm{u-\uG} \le C_1\,\estG(\uG).
  \end{equation}
%
\end{proposition}
%
This Proposition is essentially due to Babu\v ska and Miller
\cite{BabuskaMiller:87}; see also 
\cite{AinsworthOden:00,Braess:07,NoSiVe:09,Verfuerth:13}.
We point out that the lower bound in \eqref{E:IV56} is {\it oscillation-free} because
the data $\data$ is discrete; we refer to \cite{NoSiVe:09} for a
discussion of oscillation. \todo{RHN: Should we discuss this matter further? Should we
have a thorough discussion in Section \ref{S:aposteriori}?}

One serious difficulty in dealing with AFEM is that one has access to
the energy error $\enorm{u-\uG}$ only through the estimator
$\estG(\uG)$. The latter, however, fails to be monotone
because it depends on
the discrete solution $\uG\in\VG$ that changes with the mesh. 
This is tackled in the next two lemmas
\cite{CaKrNoSi:08,MoSiVe:08}.

\begin{lemma}[reduction of $\estG(V)$ with respect to $\grid$]\label{L:strict-est}
If $\lambda=1-2^{-b/d}$, then
%
\begin{equation}\label{E:strict-est}
\est_{\gridk[*]}^2 (v,\gridk[*]) \le \est_{\grid}^2 (v,\grid)
-\lambda \est_{\grid}^2 (v,\marked)
\qquad\forall v\in\V_\grid.
\end{equation}
\end{lemma}
%
\begin{proof}
To do!
\end{proof}

\begin{lemma}[Lipschitz property of $\estG(v)$ with respect to $V$]\label{L:lipschitz}
Let $\div\bA$ be the divergence of $\bA$ computed by rows, and
%
\[
    \eta_\grid(\bA,c) \definedas \max_{\in\grid}
    \big( \helm \|\div\bA\|_{L^\infty(\elm)} 
    + \|\bA\|_{L^\infty(T)} + \|c\|_{L^\infty(T)} \big).
\]
%
Then the following estimate is valid
%
  \begin{equation*}
    |\estG(v)-\estG(w)|\Cleq
    \eta_\grid(\bA,c)\enorm{v-w}
    \quad\forall v,w\in\V_\grid.
  \end{equation*}
%
\end{lemma}
%
\begin{proof}
To do!
\end{proof}

%
Upon combining Lemmas \ref{L:strict-est} and \ref{L:lipschitz}
we obtain the following crucial property.

\begin{proposition}[estimator reduction]\label{P:est-reduction}
Given $\grid\in\grids$ and a subset $\marked\subset\grid$
of marked elements, let
$\grid_*=\REFINE\big(\grid,\marked\big)$.
Then there exists a constant $\Lambda>0$, such that for all $v\in\V_\grid$,
$v_*\in\V_{\grid_*}$ and any $\delta>0$ we have
\begin{equation*}
      \est_{\grid_*}^2(v_*,\grid_*) \le
      (1+\delta)\big(\estG^2(v,\grid)-\lambda\,\estG^2(v,\marked)\big)
      +
      (1+\delta^{-1})\,\Lambda\,\eta_\grid^2(\bA,c) \,
      \enorm{v_*-v}^2.
\end{equation*}
\end{proposition}
%
\begin{proof}
To do!
\end{proof}

%-------------------------------------------------------------------------------
\subsubsection{\bf Contraction Property of $\GALERKIN$}\label{S:contraction}
%-------------------------------------------------------------------------------

A key question to ask is what is (are) the quantity(ies) that $\GALERKIN$ may
contract. In light of \eqref{L:Pythagoras},
an obvious candidate is the energy error $\enorm{u-u_k}$. 
We now show that this is in fact the
case for discrete data $\data$ provided an {\it interior node property} holds.
However, the energy error may not contract in general unless $\REFINE$ enforces
several levels of refinement, which is especially demanding in 3d. We next
present an approach that eliminates the interior
node property at the expense of a more complicated contractive quantity,
the quasi-error; see Theorem \ref{T:contraction}.

\medskip\noindent
{\bf Enforcing the interior node property.}
%
The following property was introduced by
Morin, Nochetto, and Siebert \cite{MoNoSi:00}.

\begin{definition}[interior node property]\label{D:interior-node}
The refinement $\gridk[k+1]\ge\gridk$ satisfies an interior node property
with respect to $\gridk$ if each element $T\in\marked_k$ contains
at least one node of $\gridk[k+1]$ in the interior of $T$ and of each face of
$T$.
\end{definition}
%
This property is valid upon enforcing a fixed number $b_*$ of
bisections ($b_*=3,6$ for $d=2,3$).
An immediate consequence of this property, proved in
\cite{MoNoSi:00,MoNoSi:02}, is the following {\it discrete} lower a posteriori bound:
%
\begin{equation}\label{E:lower-discrete}
C_2 \est_j(u_j,\markedk) \le \enorm{u_j-u_{j+1}}.
\end{equation}
%
\todo{This has to be proved and discussed in Section \ref{S:aposteriori}. Note the lack of
oscillation because data is discrete.}

\begin{lemma}[contraction property with interior node property]\label{L:contraction-discrete-data}
If $\gridk[j+1]$ satisfies an interior node property with respect to
$\gridk[j]$, then for $\alpha := \big(1 - \big(\theta\frac{C_2}{C_1}\big)^2\big)^{1/2} < 1$
%
\begin{equation}\label{E:simplest-contraction}
\enorm{u-u_{j+1}} \le \alpha \enorm{u-u_j},
\end{equation}
%
where $0<\theta<1$ is the parameter in \eqref{E:theta}
and $C_1 \ge C_2$ are the constants in \eqref{E:aposteriori-bounds}.
\end{lemma}
%
\begin{proof}
For convenience, we use the notation 
%
\begin{displaymath}
  e_j=\enorm{u-u_j},\ E_j=\enorm{u_{j+1}-u_j},\ \est_j=\est_j(u_j,\grid_j),\
  \est_j(\marked_j)=\est_j(u_j,\marked_j).
\end{displaymath}
%
The key idea is to use the Pythagoras equality
\eqref{E:Pythagoras},
namely $e_{j+1}^2 = e_j^2 - E_j^2$,
and show that $E_j$ is a significant portion of $e_j$. 
Since \eqref{E:lower-discrete} implies
%
$C_2 \est_j(\marked_j) \le E_j$,
%
applying D\"orfler marking \eqref{E:theta} and the upper
bound in \eqref{E:aposteriori-bounds},
we deduce
%
\begin{equation*}
E_j^2 \ge C_2^2 \theta^2 \est_j^2 \ge \Big(\theta\frac{C_2}{C_1}\Big)^2 e_j^2.
\end{equation*}
%
This is the desired property of $E_j$ and leads to \eqref{E:simplest-contraction}.
\end{proof}

We wonder whether or not the interior node property is necessary for 
\eqref{E:simplest-contraction}. We present an example, introduced
in \cite{MoNoSi:00,MoNoSi:02} to justify such a property for
constant data and $n=1$.

\begin{example}[lack of strict monotonicity]\label{nv-E:interior-node}
\rm
Let $\Omega=(0,1)^2$, $\bA=\bI, c=0, f=1$ (constant data), 
and consider the following sequences of
meshes depicted in Figure \ref{F:interior-node}.
If $\phi_0$ denotes the basis function associated with the only
interior node of the initial mesh $\grid_0$, then 
%
$u_0=u_1=\frac{1}{12}\,\phi_0$ and $u_2\neq u_1$.
%
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\textwidth]{figs/convergence/pic-4-1}
  \caption{Grids $\gridk[0]$, $\gridk[1]$, and $\gridk[2]$ of
    Example \ref{nv-E:interior-node}. The mesh $\gridk[1]$ has nodes in the
    middle of sides of $\gridk[0]$, but only $\gridk[2]$ has nodes in
    the interior of elements of $\gridk[0]$. Hence, $\gridk[2]$
    satisfies the interior node property of Definition
    \ref{D:interior-node} with respect to $\gridk[0]$ whereas
    $\grid_1$ does not.
    \label{F:interior-node}}
\end{figure}
%

\noindent
The mesh $\grid_1\ge\grid_0$ is produced by a standard $2$-step
bisection $(b=2)$ in $2d$. Since $u_0=u_1$ we conclude that the energy
error does not change 
%
$\enorm{u-u_0}=\enorm{u-u_1}$
between two consecutive steps of $\GALERKIN$ for $b=d=2$. This is no longer true provided
an interior node in each marked element is created, because then
Lemma \ref{L:contraction-discrete-data} (contraction property of $\GALERKIN$) holds.
\end{example}

\medskip\noindent
{\bf Circumventing the interior node property.}
%
Enforcing a minimal number $b_*$ of bisections, say $b_*=2,3$ for $d=2,3$, can be quite taxing
especially for $d=3$. It is clear from the preceding discussion that the energy error alone cannot
be expected to contract between consecutive iterates.
We explore next what quantity to monitor instead of the energy error in the
analysis.

%------------------------------------------------------------------------------------
\medskip\noindent
\textbf{Heuristics.}\quad According to \eqref{E:Pythagoras}, the energy
error is monotone 
%
$\enorm{u-u_{j+1}}\le\enorm{u-u_j}$,	
but the previous Example shows that strict inequality may
fail. However, if $u_{j+1}=u_j$, estimate \eqref{E:strict-est} reveals
a strict estimator reduction 
$\est_{j+1}(u_j)<\est_j(u_j)$. 
We thus expect that, for a suitable
scaling factor $\gamma>0$, the so-called \emph{quasi error}
%
\begin{equation}\label{E:quasi-error}
	\eta_j^2(u_j) := \enorm{u-u_j}^2+\gamma\,\est_j^2(u_j)
\end{equation}
%
may be contractive. This heuristics illustrates a distinct aspect of
AFEM theory, the interplay between continuous quantities such the
energy error $\enorm{u-u_j}$ and discrete ones such as the estimator
$\est_j(u_j)$: no one alone has the requisite properties to
yield a contraction between consecutive adaptive steps.


\begin{theorem}[general  contraction property]\label{T:contraction}
  Let $\theta\in (0,1]$ be the D\"orfler marking parameter,
  and $\{\grid_j,\V_j,U_j\}_{j=0}^\infty$
  be a sequence of conforming meshes, finite element spaces and
  discrete solutions created by $\GALERKIN$ for the model problem
  \eqref{strong-form}. 
%
  Then there exist constants $\gamma>0$ and $0<\alpha<1$, additionally
  depending on the number $b\ge1$ of bisections and $\theta$, such that
  for all $j\ge 0$
  \begin{equation}\label{E:contraction-prop}
    \enorm{u-u_{j+1}}^2+\gamma\,\est_{j+1}^2(u_{j+1})
    \le \alpha^2\,\Big(\enorm{u-u_j}^2+\gamma\,\est_j^2(u_j)\Big).
  \end{equation}
\end{theorem}
%
%
\begin{proof}
We split the proof into four steps and use the notation in
Lemma \ref{L:contraction-discrete-data} (contraction property with interior node property)

\step{1} The error orthogonality \eqref{E:Pythagoras} 
reads
\begin{equation}\label{E:contract-1}
  e_{j+1}^2=e_j^2-E_j^2.
\end{equation}
% 
Employing Proposition~\ref{P:est-reduction} (estimator reduction)
with $\grid=\grid_j$, $\grid_*=\grid_{j+1}$, 
$v=u_j$ and $v_*=u_{j+1}$ gives
%
\begin{equation}\label{E:contract-2}
  \est_{j+1}^2\le(1+\delta)\big(\est_j^2-\lambda
  \,\est_j^2(\marked_j)\big)+(1+\delta^{-1})\,\Lambda_0 \,E_j^2,
\end{equation}
%
where $\Lambda_0=\Lambda \eta_{\grid_0}^2(\bA,c) \ge \Lambda
\eta_{\grid_j}^2(\bA,c)$.  After multiplying
\eqref{E:contract-2} by $\gamma>0$, to be determined later, we
add \eqref{E:contract-1} and \eqref{E:contract-2} to obtain
%
\begin{align*}
  e_{j+1}^2+\gamma\,\est_{j+1}^2&\le e_j^2
  +\big(\gamma\,(1+\delta^{-1})\,\Lambda_0-1\big)\,E_j^2
  +\gamma\,(1+\delta)\,\big(\est_j^2-\lambda\,\est_j^2(\marked_j)\big).
\end{align*}
%
\step{2}
We now choose the parameters $\delta, \gamma$: let $\delta$ satisfy
%
\[
(1+\delta)\big(1-\lambda\theta^2\big) 
= 1 -\frac{\lambda\theta^2}{2},
\]
%
and $\gamma$ verify
%
\[
\gamma\,(1+\delta^{-1})\,\Lambda_0=1.
\]
%
Note that this choice of $\gamma$ yields
\begin{equation*}
  e_{j+1}^2+\gamma\,\est_{j+1}^2\le e_k^2
  +\gamma\,(1+\delta)\,\big(\est_j^2-\lambda\,\est_j^2(\marked_j)\big).
\end{equation*}
% 
\step{3}
We next employ D\"orfler Marking \eqref{E:theta}, namely 
$\est_j(\marked_j)\ge\theta\est_j$, to deduce
%
\begin{equation*}
  e_{j+1}^2+\gamma\,\est_{j+1}^2
  \le
  e_j^2
  + \gamma (1+\delta)(1-\lambda\theta^2)\est_j^2
\end{equation*}
%
which, in conjunction with the choice of $\delta$, gives
%
\begin{equation*}
  e_{j+1}^2+\gamma\,\est_{j+1}^2 
  \le 
  e_j^2
  + \gamma \bigg(1-\frac{\lambda\theta^2}{2}\bigg)\est_j^2
  = e_j^2 - \frac{\gamma\lambda\theta^2}{4}\est_j^2
  + \gamma \bigg(1-\frac{\lambda\theta^2}{4}\bigg)\est_j^2.
\end{equation*}
%
\step{4} Finally, the upper bound in \eqref{E:aposteriori-bounds}, namely
\begin{math}
  e_J\le C_1\,\est_j,
\end{math}
%
implies that
%
\begin{displaymath}
  e_{j+1}^2+\gamma\,\est_{j+1}^2 \le 
  \bigg(1-\frac{\gamma\lambda\theta^2}{4C_1^2}\bigg) e_j^2
  + \gamma \bigg(1-\frac{\lambda\theta^2}{4}\bigg) \est_j^2.
\end{displaymath}
%
This in turn leads to
%
\begin{displaymath}
  e_{j+1}^2+\gamma\,\est_{j+1}^2 
  \le  \alpha^2
  \big(e_j^2 +\gamma\,\est_j^2\big),
\end{displaymath}
%
with
%
$\alpha^2 \definedas \max \big\{1-\frac{\gamma\lambda\theta^2}{4C_1^2},
  1-\frac{\lambda\theta^2}{4} \big\}<1$,
%
and thus concludes the theorem. 
\end{proof}

\begin{remark}[basic ingredients]
\rm 
  This proof solely uses D\"orfler
  marking \eqref{E:theta}; 
  Pythagoras identity \eqref{E:Pythagoras}; the a posteriori
  upper bound in \eqref{E:aposteriori-bounds}; and Proposition~\ref{P:est-reduction} (estimator
  reduction). The proof does not use the
  lower bound in \eqref{E:aposteriori-bounds}. 
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\bf Convergence for General Data}\label{S:general-data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now remove the restriction of Section \ref{S:discrete-data} of discrete data
$\data \in \X_{\wh\grid}$ and allow for general data $\data = (\bA,c,f) \in\X$,
where $\X$ and $\X_{\wh\grid}$ are defined in \eqref{E:space-data} and \eqref{E:space-discrete-data}.


%-------------------------------------------------------------------------------
\subsubsection{\bf Perturbation estimate}\label{S:perturbation}
%-------------------------------------------------------------------------------
%
We first quantify the effect of perturbing data from $\data$ to $\wh\data$ in the space
%
\[
D(\Omega) = L^\infty(\Omega; \R^{d\times d}) \times W^{-s}_q(\wh\grid) \times H^{-1}(\Omega).
\]
%
The use of the max-norm for the diffusion coefficient $\bA$ 
entails piecewise uniform continuity
of $\bA$ over a generic mesh $\grid\in\grids$. In Section \ref{S:discontinuous-coeffs} we
will tackle the important case of coefficients $(\bA,c)$ with discontinuities not aligned with $\grid$.

\begin{lemma}[continuous dependence on data] \label{L:perturbation}
Let $\data=(A,c,f) \in \X$ such that $A\in M(\alpha_1,\alpha_2$ and $c\in R(c_1,c_2)$. Let
$\wh\data=(\wh\bA,\wh{c},\wh{f})\in\X_{\wh\grid}$ be an approximation of $\data$ such that
$(\wh\bA,\wh{c})$ satisfy \eqref{E:structural-assumption} and \eqref{E:wh-alpha}.
%
For $d < q  \leq \infty$ and $1-d/q \leq s \leq 1$, there holds
%
\begin{equation}\label{E:perturbation}
 \| \nabla (u- \hu) \|_{L^2(\Omega)} \le C(\data,\Omega) \, \|\data-\hdata\|_{D(\Omega)}
\end{equation}
where the constant $C(\data,\Omega)$ also depends on the shape-regularity of $\grids$, $q$ and $s$.
\end{lemma}
%
\begin{proof}
Subtracting the weak formulations \eqref{weak-form} for $u$ and \eqref{E:perturbed-pb} for $\wh{u}$,
and reordering, we easily obtain for any $v \in H^1_0(\Omega)$
$$
\int_\Omega \nabla v \cdot \hA \nabla (u-\hu) + \hc v (u-\hu) =
\int_\Omega \nabla v \cdot (\hA-A) \nabla u + (\hc-c) v u + \langle f-\hf,v \rangle.
$$
%
We choose $v = u-\hu \in H^1_0(\Omega)$ and invoke \eqref{E:enorm-Vnorm-wh} with
$c_{\wh\B}=\frac{\alpha_1}{4}$ to deduce
%
\begin{equation*}\label{e:perturb_coerc}
\frac{\alpha_1}{4} \| \nabla v \|_{L^2(\Omega)}^2 \leq \int_\Omega \nabla v \cdot (\hA-A) \nabla u + (\hc-c) v u + \langle f-\hf,v \rangle.
\end{equation*}
%
We estimate separately each term separately, starting with the first and last terms
%
\begin{equation*}\label{e:perturb_a}
\int_\Omega \nabla v \cdot (\hA-A) \nabla u \leq \| \hA-A  \|_{L^\infty(\Omega)} \| \nabla u \|_{L^2(\Omega)} \| \nabla v \|_{L^2(\Omega)}
\end{equation*}
and
\begin{equation*}\label{e:perturb_f}
\langle f-\hf,v \rangle \leq \| f - \hf \|_{H^{-1}(\Omega)} \| \nabla v \|_{H^1(\Omega)}.
\end{equation*}
%
For the reaction term, we invoke the duality pairing $W^s_{q'}-W^{-s}_{q}$ for every element $T\in\grid$,
where $q' \geq 1$ is given by $1/q+1/q'=1$ (as usual we identify $L^2$ with its dual) to obtain
\begin{equation*}\label{e:perturb_reac}
\int_\Omega (\hc-c) v u \lesssim  \left(\sum_{T\in \grid} \| \hc -c \|_{W^{-s}_q(T)}^q\right)^{1/q} \| vu \|_{W^{s}_{q'}(\Omega)}.
\end{equation*}
%
We now estimate $\| vu \|_{W^{s}_{q'}(\Omega)} \lesssim \| vu \|_{W^{1}_{p'}(\Omega)}$ for $p'\ge1$
given by the relation
%
\[
1-\frac d{p'} = \textrm{sob}(W^1_{p'})  = \textrm{sob}(W^s_{q'})= s - \frac d{q'}.
\]
%
\todo{RHN: reference for the embedding with equality of Sobolev numbers.}
Note that $p' \geq 1$ thanks to the restrictions $s\geq 1-d/q$ and $q>d$.
On the other hand, $p'<2$ because $s\le1$, $q>d\ge2$ and
$$
d\left(\frac 1 2 - \frac 1 {p'}\right) = s-1 + d\left(\frac 12-\frac 1{q'}\right) = s-1 - d \left(\frac 1 2 - \frac 1{q}\right) < 0.
$$
%
This implies the estimate
%
\begin{equation*}\label{e:prod_estimate} 
\| vu \|_{W^{s}_{q'}(\Omega)} \lesssim \| vu \|_{W^{1}_{p'}(\Omega)} \lesssim \left( \| u v\|_{L^{p'}(\Omega)}+ \| u\nabla v \|_{L^{p'}(\Omega)} + \| v \nabla u \|_{L^{p'}(\Omega)} \right)
\end{equation*}
%
whence
%
\begin{equation*}\label{e:prod_ws}
\| vu \|_{W^{s}_{q'}(\Omega)} \lesssim \| u \|_{L^2(\Omega)}\| v \|_{L^{r}(\Omega)}+ \| \nabla v\|_{L^2(\Omega)} \| u \|_{L^{r}(\Omega)} + \| v \|_{L^r(\Omega)} \| \nabla u \|_{L^{2}(\Omega)},
\end{equation*}
where $r$ is chosen so that $\frac 1 r + \frac 1 2 = \frac 1{p'}$ or equivalently $r=\frac{2p'}{2-p'} \in [2,\infty)$. 
Furthermore, notice that
$$
1-\frac d 2  = \textrm{sob}(H^1) > \textrm{sob}(L^r) = - \frac d r
$$
because
$$
1- d\left(\frac 1 2 - \frac 1 r \right) = 1- d\left(1 - \frac 1 {p'}\right) = 2-s - d \left(1 - \frac 1 {q'}\right) =2-s - \frac{d}{q} \ge 1 - \frac{d}{q} >  0.
$$
%
Consequently, $H^1(\Omega)$ continuously embeds in $L^r(\Omega)$ and together with the Poincar\'e inequality
\eqref{E:Poincare} gives the estimate
$$
\| vu \|_{W^{s}_{q'}(\Omega)} \lesssim  \| \nabla v\|_{L^2(\Omega)} \| \nabla u \|_{L^{2}(\Omega)}.
$$
%
We finally observe that the factor $\| \nabla u \|_{L^{2}(\Omega)}$ appears in the estimates
of the coefficients $(\bA,c)$ and reflects the multiplicative nature of these terms. This
factor can be further bounded in terms of $\data$, namely
$\| \nabla u \|_{L^{2}(\Omega)} \le \alpha_1^{-1} \|f\|_{H^{-1}(\Omega)}$.
This in conjunction with the preceding estimates yields the assertion \eqref{E:perturbation}.
\end{proof}

A natural choice for the parameters $(s,q)$ in Lemma \ref{L:perturbation} (continuous dependence on data)
is $q=\infty$ and $s=1$, but this would prevent the reaction coefficient $c$ from being discontinouus
within elements. We will discuss this matter further in Section \ref{S:data-approx}, along with the
treatment of discontinuous coefficients $(\bA,c)$.

In view of Theorem \ref{T:contraction} (general contraction property),
it is also important to quantify the effect of 
changing discrete data in the error estimator. To this end, for $i=1,2$ let $(\wh\grid_i,\wh\data_i)$
be two mesh-discrete data pairs generated by $\DATA$ with $\wh\grid_2$ being a conforming refinement of
$\wh\grid_1$, i.e. $\wh\grid_2 \ge \wh\grid_1$.

\begin{lemma}[perturbation of error estimator]\label{L:perturbation-estimator}
Let $\grid_2\ge\grid_1$ be conforming refinements of $\wh\grid_2,\wh\grid_1$, and let
$u_i \in \V_i = \V_{\grid_i}$ be the corresponding Galerkin solutions of \eqref{E:galerkin}
with data $\wh\data_i$. Then
the estimators $\est_i(u_i)=\est_{\grid_i}(u_i)$ satisfy
%
\begin{equation}\label{E:perturbation-estimator}
\est_2(u_2) \le \est_1(u_1) + \wh{C}_1 \|\wh\data_2-\wh\data_1\|_{D(\Omega)} + \wh{C}_2 |u_2-u_1|_{H^1_0(\Omega)}
\end{equation}
%
where the constants $\wh{C}_1,\wh{C}\wh{C}_2$ depend on data, the shape regularity of $\grids$ and the
polynomial degree $n$.
\end{lemma}
%
\begin{proof}
Let $\wh\data_i = (\wh\bA_i,\wh{c}_i,\wh{f}_i) \in \X_{\wh\grid_i}$ and remove the hats for
simplicity of notation. We recall the expression \eqref{E:discrete-load} and use the
symbol $f$ the denote both the absolutely continuous term $q_T$ for $T\in\wh\grid$ and
the singular term $q_F$ for $F\in\wh\faces$, with respect to Lebesgue measure.
We now proceed in several steps.

\step{1} {\it Decomposition of the residuals}: In view of the definitions \eqref{E:residuals}
of the interior residual $r(u_2)$ and jump residual $j(u_2)$, we can rewrite them as follows:
%
\begin{align*}
r(u_2) &= f_2 + \div \big( \bA_2 \nabla u_2 \big) - c_2 u_2
\\
& = r(u_1) + \div \big(\bA_1 (\nabla (u_2-u_1)  \big)  + c_1  \big( u_2-u_1 \big)
\\
& + \big(f_2 - f_1 \big) + \div \big( (\bA_2-\bA_1) \nabla u_2 \big) + \big(c_1 - c_2 \big) u_2,
\end{align*}
%
and
%
\begin{align*}
j(u_2) &= \big( [\bA_2 \nabla u_2] + f_2 \big)\cdot\nu
\\
& = j(u_1) + \big[\bA_1 \nabla (u_2-u_1)  \big]\cdot\nu
+ \big(f_2 - f_1 \big)\cdot\nu + \big[ (\bA_2-\bA_1) \nabla u_2 \big]\cdot\nu.
\end{align*}
%
Since $\est_2(u_2)$ is a weighted $\ell^2$-norm for the discrete quantities $r(u_2)|_T$ and
$j(u_2)|_T$ for $T\in\grid_2$, applying the triangle inequality together with the fact that
the local meshsize decreases from $\grid_1$ to $\grid_2$, because $\grid_2\ge\grid_1$, we deduce
%
\begin{align*}
\est_2(u_2) = \bigg( \sum_{T\in\grid_2} h_T^2 \|r(u_2)\|^2_{L^2(T)} + h_T \|j(u_2)\|^2_{L^2(\partial T)}\bigg)^{\frac12}
\le \est_1(u_1) + \sum_{i=1}^5 R_i,
\end{align*}
%
where
%
\begin{align*}
R_1^2 & = \sum_{T\in\grid_2} h_T^2 \| \div \big(\bA_1 (\nabla (u_2-u_1)  \big)  + c_1  ( u_2-u_1 ) \|_{L^2(T)}^2,
\\
R_2^2 & = \sum_{T\in\grid_2} h_T \| [\bA_1 \nabla (u_2-u_1)  ]\cdot\nu \|_{L^2(\partial T)}^2,
\\
R_3^2 &= \sum_{T\in\grid_2} h_T^2 \| f_2 - f_1 \|_{L^2(T)}^2 + h_T \| (f_2 - f_1)\cdot\nu \|_{L^2(\partial T)}^2 ,
\\
R_4^2 &= \sum_{T\in\grid_2} h_T^2 \| \div [(\bA_2-\bA_1) \nabla u_2 ]  \big)  + (c_2-c_1) u_2 \|_{L^2(T)}^2,
\\
R_5^2 &= \sum_{T\in\grid_2} h_T \|(\bA_2-\bA_1) \nabla u_2 \cdot\nu \|_{L^2(\partial T)}^2.
\end{align*}

\step{2} {\it Estimate for $R_1$ and $R_2$}: Since $\bA_1$, $u_2$ and $u_1$ are piecewise polynomials
over $\grid_2$, and $(\bA_1,c_1)$ satisfy \eqref{E:structural-assumption},
we resort to trace and inverse inequalities to obtain
%
\[
R_1^2 + R_2^2 \lesssim \sum_{T\in\grid_2} h_T^2 \|D^2_h(u_2 - u_1)\|_{L^2(\omega_T)}^2
+ \|u_2 - u_1\|_{H^1(\omega_T)}^2 \lesssim |u_2 - u_1|_{H^1_0(\Omega)}^2,
\]
%
where $D_h^2$ stands for the broken Hessian and $\omega_T$
for the set of elements of $\grid_2$ containing $\partial T$.
The last inequality is a consequence of the finite overlapping property of $\{\omega_T\}_{T\in\grid_2}$
and Poincar\'e inequality \eqref{E:Poincare}. The hidden constant depends on the shape regularity
of $\grids$ and the polynomial degree $n$.

\step{3} {\it Estimate of $R_3$}: We invoke Corollary \ref{L:dual-norms} (computing dual norms of
discrete functionals) to infer that
%
\todo{Does Corollary \ref{L:dual-norms} apply directly to $f_2-f_1$, which are defined on different
meshes, or has to be extended?}
%
\[
R_3^2 \lesssim \sum_{z\in\nodes_2} \|f_2 - f_1\|_{H^{-1}(\omega_z)}^2 \approx
\|f_2 - f_1\|_{H^{-1}(\Omega)}^2.
\]
%

\step{4} {\it Estimate of $R_4$ and $R_5$}: We again employ the fact that
$\bA_1,\bA_2$, and $u_2$ are piecewise polynomials over $\grid_2$, and combine trace and
inverse inequalities to get
%
\[
R_4^2 + R_5^2 \lesssim \sum_{T\in\grid_2} \|\nabla u_2\|_{L^2(\omega_T)} \Big(\|\bA_1 -\bA_2\|_{L^\infty(\omega_T)}
 + \|c_1-c_2\|_{W^{-s}_q(T)}\Big),
\]
%
upon arguing similarly to Lemma \ref{L:perturbation} (continuous dependence on data)
for $d<q\le\infty$ and $1-d/q\le s \le 1$.

\step{5} {\it Conclusion}: Finally, realizing that
$\|\nabla u_2\|_{L^2(\omega_T)} \le \alpha_2^{-1} \|f_2\|_{H^{-1}(\Omega)}$ and recalling the definition
\eqref{E:approx-space} on $D(\Omega)$, the preceding
estimates lead to the assertion.
\end{proof}

%-------------------------------------------------------------------------------
\subsubsection{\bf Module $\DATA$}\label{S:DATA}
%-------------------------------------------------------------------------------
%
In this section we briefly discuss the structure of $\DATA$ in the simplest case of
polynomial degree $n=1$.
We start with the element error estimators for $(\bA,c)$. Let $s=1, q = \infty$ and
for all $T\in\wh\grid$ let
%
\begin{equation}\label{E:zeta-Ac-loc}
\zeta_{\wh\mesh}(T; \bA) := 
\Vert \bA - \wh \bA\Vert_{L^\infty(T)} \,,
\quad
\zeta_{\wh \mesh}(T; c)  := 
h_T \|  c-\wh{c} \|_{L^{\infty}(T)}\,,
\end{equation}
%
where $(\wh \bA,\wh c)$ are the element meanvalues of $(\bA,c)$, namely
%
\begin{equation}\label{E:meanvalues}
\wh \bA := \frac{1}{|T|} \int_T \bA,
\quad
\wh c := \frac{1}{|T|} \int_T c,
\quad\forall T\in \wh\grid
\end{equation}
%
which satisfy $\bA \in M(\alpha_1,\alpha_2), c\in R(c_1,c_2)$ defined in \eqref{E:structural-assumption}.
Therefore, the $L^2$-projection on piecewise constants over $\wh\grid$ satisfies the side conditions
in \eqref{E:structural-assumption} without changing the original range of parameters. The $L^2$-projection
on piecewise polynomials of degree $n-1$ for $n>1$ would not satisfy \eqref{E:structural-assumption}
and must be modified nonlinearly; this is fully discussed in Section \ref{S:data-approx}. This explains
our choice $n=1$.

The approximation of a load $f\in H^{-1}(\Omega)$ is trickier for several reasons. First the norm in
$H^{-1}(\Omega)$ is nonlocal. Lemma \ref{L:residual-loc} (localization of residual norm) explains how
to localize it to stars $\{\omega_z\}_{z\in\wh\nodes}$. Therefore, we consider star error
estimators
%
\begin{equation}\label{E:zeta-star}
\zeta_{\wh\mesh}(z; f) := 
\Vert f - P_{\wh\grid} f\Vert_{H^{-1}(\omega_z)}
\quad\forall z\in\wh\nodes.
\end{equation}
%
The second issue at stake is that without further assumptions on $f$, it is not possible to
evaluate or bound the right hand side of \eqref{E:zeta-star}. In Section \ref{S:data-approx} we
will consider surrogates, namely classes of loads with structural properties that allow
for estimation of \eqref{E:zeta-star} and yet are relevant in practice. This includes the usual
case $f\in L^2(\Omega)$ that leads to the standard weighted $L^2$-element error estimator
%
\begin{equation}\label{E:weighted-L^2}
\zeta_{\wh\mesh}(T; f) := 
h_T \Vert f - \wh f\Vert_{L^2(T)}
\quad\forall T\in\wh\grid
\end{equation}
%
where $\wh{f}$ stands for the element meanvalue defined in \eqref{E:meanvalues}.

The global data error estimators for the coefficients $(\bA,c)$ are given by
%
\begin{equation}\label{E:zeta-Ac-global}
\zeta_{\wh\mesh}(\bA) := \max_{T\in\wh\grid} \zeta_{\wh\mesh}(T; \bA),
\quad
\zeta_{\wh\mesh}(c) := \max_{T\in\wh\grid} \zeta_{\wh\mesh}(T; c),
\end{equation}
%
which accumulate in $\ell^\infty$. In contrast, the global error estimator for $f$
%
\begin{equation}\label{E:zeta-f-global}
\zeta_{\wh\mesh}(f) := \bigg(\sum_{z\in\wh\nodes} \zeta_{\wh\mesh}(z; f)^2 \bigg)^{\frac{1}{2}}
\end{equation}
%
accumulates in $\ell^2$. This fact is responsible for two different procedures, greedy and
pseudo-greedy, used below to mark elements. The total data error estimator is
%
\begin{equation}\label{E:total-data-est}
\zeta_{\wh \mesh}(\data) := 
\zeta_{\wh \mesh}(A) +
\zeta_{\wh \mesh}(c) +
\zeta_{\wh \mesh}(f) \,.
\end{equation}
%

The call $[\wh\grid,\wh\data]=\DATA (\grid,\data,\tau)$ consists of iterations of
the following loop
%
\begin{equation}\label{E:paradigm_data}
\PROJECT 
\longrightarrow \,
\ESTIMATEDATA 
\longrightarrow \,
\MARKDATA
\longrightarrow \,
\REFINE .
\end{equation}
%
This call produces a sequence of conforming meshes $\{\widehat\mesh_j\}_{j\geq 0}$, with $\widehat\mesh_0=\mesh$, and associated discrete data $\widehat\data_j = (\widehat{A}_j,\widehat{c}_j,\widehat{f}_j)$ w.r.t. $\widehat\mesh_j$, that approximates the exact 
 data $\mathcal{D}$ until a $j \geq 0$ is found that satisfies $\zeta_{\widehat\mesh_j}(\data) \leq \tau$. 
%
The modules in \eqref{E:paradigm_data} are defined as follows:

\medskip
\begin{itemize}%[$\bullet$]
\item $[\widehat\data]=\texttt{PROJECT}(\mesh, \data)$ computes the local components \eqref{E:meanvalues}
and \eqref{E:zeta-star} of $\widehat \data = (\widehat{A},\widehat{c},\widehat{f})$ over $\mesh$;
\item $[\{\zeta_\mesh(\, \cdot \, ;A)\}, \, 
\{\zeta_\mesh(\, \cdot \, ;c)\}, \,
\{\zeta_\mesh(\, \cdot \, ;f)\}]=\ESTIMATEDATA (\mesh, \data, \widehat\data)$ computes the local data error estimators \eqref{E:zeta-Ac-loc} and \eqref{E:zeta-star} on the mesh $\mesh$;
\item $[\mathcal{M}_{\data}] = \MARKDATA (\mesh, \{\zeta_\mesh(\, \cdot \, ;A)\}, \, 
\{\zeta_\mesh(\, \cdot \, ;c)\}, \,
\{\zeta_\mesh(\, \cdot \, ;f)\},  \theta, \tau)$  implements  the following marking criteria:
for the coefficients $(\bA,c)$ we apply the {\it greedy} strategy that selects
%
\[
\mathcal{M}_A := \big\{T\in \mesh \, :\,  \zeta_\mesh(T;\bA) \geq \tfrac13 \tau \big\} \,,
\quad
\mathcal{M}_c := \big\{T \in \mesh \, :\,  \zeta_\mesh(T;c) \geq \tfrac13 \tau \big\} \,.
\]
For the load term  $f$, which accumulates in $\ell^2$ rather than $\ell^\infty$, we first check if $\zeta_\mesh(f) \geq \tfrac13 \tau$, and if so we apply a {\it pseudo-greedy} strategy that, given a parameter $\theta \in (0,1)$,  selects
\begin{equation}
\label{eq:pseudogreedy-data}
\mathcal{M}_f := \{z \in \nodes \, :\,  \zeta_\mesh(z;f) \geq \theta \, \max_{z' \in \nodes}  \zeta_\mesh(z';f) \,.
%\tfrac19 \theta \varepsilon^2
%\leq \theta \zeta_{\mesh}^2 (f) \leq 
%\sum_{E \in \mathcal{M}_f} \zeta_{\mesh}^2(E; f) \,.
\end{equation} 
%%
%%
 Finally, we let the marked set be $\mathcal{M}_\data := \mathcal{M}_A \cup \mathcal{M}_c \cup \mathcal{M}_f$. In Section \ref{S:data-approx}, we assess the optimality properties of both greedy and pseudo-greedy algorithms.
 
\item $[\widehat\mesh]=\REFINE (\mesh, \mathcal{M}_\data)$ produces a conforming refinement $\widehat\mesh$ of $\mesh$, obtained by newest-vertex bisection of all the elements in $\mathcal{M}_\data$ and, possibly, some other elements.  This is the same procedure described in Section \ref{S:bisection}, but applied with $\mathcal{M}$ replaced by $\mathcal{M}_\data$.
\end{itemize}

\medskip
Altogether, the call $[\wh\grid,\wh\data]=\DATA (\grid,\data,\tau)$ creates a conforming refinement
$\wh\grid$ of $\grid$ and discrete data $\wh\data$ over $\wh\grid$ satisfying the error estimate
\eqref{E:error-data}, namely
%
\[
\|\data - \wh\data\|_{D(\Omega)} \le \tau.
\]
%
We make the following regularity assumption on data $\data$ and about the performance of the
procedure $\MARKDATA$. This is what we need for this and next sections and postpone a full discussion
of both issues to Section \ref{S:data-approx}.

\begin{assumption}[complexity of $\DATA$]\label{A:complexity-data}
Given a real number $0 < s\le \frac{n}{d}$, we say that data $\data$ belongs to the approximation
class $\D_s$ if for every integer $N \ge \#\grid_0$ there is a mesh $\wh\grid\in\grids$ with
cardinality $\#\wh\grid\le N$ such that
%
\begin{equation}\label{E:class-data}
\|\data-\wh\data\|_{D(\Omega)}\le C N^{-s},
\end{equation}
%
where $C>0$ is independent of $N$, and denote by $|\data|_s$ the smallest constant $C$.
%
Given $\tau>0$, the procedure $\MARKDATA$ marks a number of elements $\#\marked$
satisfying
%
\begin{equation}\label{E:complexity-data}
\# \marked \lesssim |\data|_s \tau^{-\frac{1}{s}}.
\end{equation}
\end{assumption}

In view of Lemma \ref{L:perturbation} (continuous dependence on data), there exists a constant
$C_D$ depending on $\data, \Omega$, and the shape regularity of $\grids$, such that the exact solutions $u$
and $\hu$ of \eqref{strong-form} and \eqref{E:perturbed-pb}, corresponding to data $\data$ and $\wh\data$,
satisfy the error estimate
%
\begin{equation}\label{E:error-DATA}
\enorm{u-\hu} \le C_D \tau.
\end{equation}


%-------------------------------------------------------------------------------
\subsubsection{\bf Computational cost of $\GALERKIN$}\label{S:cost-galerkin}
%-------------------------------------------------------------------------------
%
We now investigate the number of iterations within $\GALERKIN$, which dictate its computational
cost. We point out that at iteration $k-1\ge0$ the output of $\GALERKIN$, and thus of
$\AFEM$, satisfies
%
\begin{equation}\label{E:output-galerkin}
\est_k(u_k) \le \eps_{k-1}
\quad\Rightarrow\quad
\enorm{u_k - \hu_{k-1}} \le C_1 \eps_{k-1}
\end{equation}
%
according to \eqref{E:aposteriori-bounds}, where $\hu_{k-1}\in H^1_0(\Omega)$ is the exact
solution with discrete data $\wh\data_{k-1}$. The next iteration $k$ of $\AFEM$ calls $\DATA$,
which in turn changes the discrete data from $\wh\data_{k-1}$ to $\wh\data_k$
and mesh from $\grid_k$ to $\wh\grid_k$. The pair $(\wh\grid_k,\wh\data_k)$ determines
the first Galerkin solution $u_{k,0}\in\V_{k,0}=\V_{\wh\grid_k}$ of $\GALERKIN$
and corresponding estimator $\est_{\grid_{k,0}}(u_{k,0},\wh\data_k)$ with $\grid_{k,0}=\wh\grid_k$.
The reduction of $\est_{\grid_{k,j}}(u_{k,j},\wh\data_k)$ for $j\ge 1$ dictates the
number of iterations of $\GALERKIN$. We examine this next.

\begin{proposition}[computational cost of $\GALERKIN$]\label{P:cost-galerkin}
For any $k\in\N$, the number of subiterations $J_k$ inside a call to $\GALERKIN$ at
iteration $k$ of $\AFEM$ is bounded independently of $k$.
\end{proposition}
%
\begin{proof}
We exploit the fact that $\GALERKIN$ contracts the quasi-error
$\eta_{k,j}(u_{k,j})=\eta_{\grid_{k,j}}(u_{k,j},\wh\data_k)$
defined in \eqref{E:quasi-error},
namely if $(\grid_{k,j},u_{k,j})$ is the output of the $j$-th loop OF $\GALERKIN$ at step $k$
of $\AFEM$, then
%
\begin{equation}\label{E:contraction}
\eta_{k,j}(u_{k,j}) \le \alpha \, \eta_{k,j-1}(u_{k,j-1}) \quad\forall j\ge1,
\end{equation}
%
where $0<\alpha<1$ 
according to Theorem \ref{T:contraction} (general contraction property). We can assume that
$\est_{\grid_{k,0}}(u_{k,0},\wh\data_k)>\eps_k$ for otherwise $\GALERKIN$
would not be called. We first prove that $\eta_{k,0}(u_{k,0})\lesssim\eps_k$ and next argue that $J_k$
is bounded uniformly in $k$. We proceed in several steps.

\smallskip
\step{1} {\it Bound on $\enorm{u_{k,0}-\hu_k}$}: Since $u_k\in\V_k\subset\V_{k,0}=\V_{\wh\grid_k}$,
and the Galerkin
solution $u_{k,0}\in\V_{k,0}$ minimizes the energy norm relative to $\hu_k$, we deduce
%
\[
\enorm{u_{k,0}-\hu_k} \le \enorm{u_k-\hu_k}
\le \enorm{u_k-\hu_{k-1}} + \enorm{\hu_{k-1}-\hu_k}
\]
%
Invoking the a posteriori upper bound in \eqref{E:aposteriori-bounds}, and the termination condition
of $\GALERKIN$ at step $k-1$, we obtain
%
\[
\enorm{u_k-\hu_{k-1}} \le C_1 \est_{\grid_k}(u_k,\wh\data_{k-1}) \le C_1 \eps_{k-1} = 2C_1 \eps_k.
\]
%
On the other hand, combining \eqref{E:enorm-Vnorm-wh} with \eqref{E:perturbation} of
Lemma \ref{L:perturbation} (continuous dependence on data), we arrive at
%
\[
\enorm{u-\hu_k} \le \sqrt{C_{\wh\B}} |u-\hu_k|_{H^1_0(\Omega)}
\le C_3 \|\data-\wh\data_k\|_{D(\Omega)} \le C_3 \eps_k,
\]
%
where we have used that the output $\wh\data_k$ of $\DATA$ satisfies $\|\data-\wh\data_k\|_{D(\Omega)}
\le \omega \eps_k$ with $\omega\le1$ and $C_3=\sqrt{C_{\wh\B}}\,C(\data,\Omega)$.
The triangle inequality thus yields
%
\[
\enorm{\hu_{k-1}-\hu_k} \le \enorm{u-\hu_{k-1}} + \enorm{u-\hu_k} \le C_3(\eps_{k-1}+\eps_k)
= 3C_3 \eps_k,
\]
%
whence
%
\[
\enorm{u_{k,0}-\hu_k} \le \big(2C_1 + 3C_3 \big) \eps_k = C_4 \eps_k.
\]

\step{2} {\it Bound on $\est_{\grid_{k,0}}(u_{k,0},\wh\data_k)$}: Since $\grid_{k,0}=\wh\grid_k\ge\grid_k$,
applying Lemma \ref{L:perturbation-estimator} (perturbation of error estimator) gives
%
\[
\est_{\grid_{k,0}}(u_{k,0},\wh\data_k)
\le \est_{\grid_k}(u_k,\wh\data_{k-1}) + \wh{C}_1 \|\wh\data_k-\wh\data_{k-1}\|_{D(\Omega)}
+ \wh{C}_2 |u_{k,0} - u_k|_{H^1_0(\Omega)}. 
\]
%
When $\GALERKIN$ stops $\est_{\grid_k}(u_k,\wh\data_{k-1})\le\eps_{k-1}$, whereas when $\DATA$ does it
%
\[
\|\data-\wh\data_k\|_{D(\Omega)} \le \omega\eps_k,
\]
%
whence
%
\[
\|\wh\data_k-\wh\data_{k-1}\|_{D(\Omega)} \le \eps_k+\eps_{k-1} = 3\eps_k.
\]
%
On the other hand, using \eqref{E:enorm-Vnorm-wh} together with the estimate from Step 1 implies
%
\[
|u_{k,0} - u_k|_{H^1_0(\Omega)} \le c_{\wh\B}^{-1/2} \enorm{u_{k,0} - u_k}
\le 2 c_{\wh\B}^{-1/2} \enorm{u_k - \hu_k} \le 2 c_{\wh\B}^{-1/2} \big(2C_1 + 3C_3 \big) \eps_k.
\]
%
Altogether, we have proved the existence of a constant $C_5$ such that
%
\[
\est_{\grid_{k,0}}(u_{k,0},\wh\data_k) \le C_5 \eps_k.
\]

\step{3} {\it Bound on $J_k$}:
The first Galerkin solution $u_{k,0}$ satisfies
%
\[
\eta_{k,0}^2 (u_{k,0}) = \enorm{u_{k,0}-\hu_k}^2+\gamma \est_{\grid_{k,0}}^2(u_{k,0},\wh\data_k)
\le \big( C_4 + \gamma C_5 \big) \eps_k^2.
\]
%
In view of \eqref{E:contraction}, each succesive iterate $(\grid_{k,j},u_{k,j})$ of $\GALERKIN$
obeys the relation
%
\[
\eta_{k,j}(u_{k,j}) \le \alpha^j \eta_{k,0}(u_{k,0})
\le \alpha^j \big( C_4 + \gamma C_5 \big)^{\frac12} \eps_k,
\]
%
whence
%
\[
\est_{\grid_{k,j}}(u_{k,j},\wh\data_k) \le \alpha^j \Big(\frac{C_4 + \gamma C_5}{\gamma}\Big)^{\frac12} \eps_k
= C_6 \, \eps_k
\]
%
$\GALERKIN$ stops once $\est_{\grid_{k,j}}(u_{k,j},\wh\data_k)\le\eps_k$ and $J_k$ is the smallest
such $j$. Hence
%
\[
\eps_k < \est_{\grid_{J_k-1}}(u_{k,J_k-1},\wh\data_k) \le
\alpha^{J_k-1} C_6 \, \eps_k.
\]
%
This implies the asserted bound $J_k \le 1 + \frac{\log C_6}{\log \alpha^{-1}}$ uniform in $k$.
\end{proof}

%-------------------------------------------------------------------------------
\subsubsection{\bf Realization of AFEM}\label{S:realization-AFEM}
%-------------------------------------------------------------------------------
%
Given an initial tolerance $\eps_0>0$, a target tolerance $\tol$ and initial mesh $\mesh_0$,
as well as a safety parameter $\omega \in (0,1]$, AFEM consists of the two-step algorithm:

\medskip
\begin{algotab}
  \>  $[\mesh, u_\mesh]=\AFEM (\mesh_0, \varepsilon_0, \omega, \tol)$
  \\
  \>  $\quad  k= 0$ 
  \\
  \>  $\quad \text{while } \varepsilon_k >  \tfrac12 \tol$
  \\
  \>  $\quad \quad  [\widehat\mesh_{k},\widehat{\data}_{k}]=\DATA \, (\mesh_k, \data, \omega \, \varepsilon_k) $ 
  \\
  \>  $\quad \quad [\mesh_{k+1},u_{k+1}]=\GALERKIN \, (\widehat{\mesh}_{k},\widehat{\data}_{k},\varepsilon_k)$ 
  \\
  \>  $\quad \quad  \varepsilon_{k+1}=\tfrac12 {\varepsilon_k}$
  \\
  \>  $\quad \quad  k \leftarrow k+1$
  \\
  \>  $\quad  \text{end while }$
  \\
  \>  $\quad  \text{return} \, (\mesh_k, u_k)$
\end{algotab}
\medskip
%

\begin{proposition}[convergence of $\AFEM$]\label{P:convergence-AFEM}
For each $k\ge0$ the modules $\DATA$ and $\GALERKIN$ converge in a finite number of iterations, the
latter independent of $k$
Moreover, there exists a constant $C_*$ depending solely on $\mesh_0$ such that the output of $[\mesh_{k+1},u_{k+1}]=\GALERKIN \, (\widehat{\mesh}_{k},\widehat{\data}_{k},\varepsilon_k)$ satisfies
%
$\enorm{{u} -u_{k+1}} \leq C_* \varepsilon_k$ for all $k \geq 0$.    
%
Therefore, $\AFEM$ stops after $K<1+\frac{\log\frac{\eps_0}{\tol}}{\log2}$ iterations and delivers
%
\begin{equation*}
  \enorm{ u -u_{K+1} } \leq C_* \tol.
\end{equation*}   
%
\end{proposition}
%
\begin{proof}
In view of Assumption \eqref{A:complexity-data} (complexity of data) the module $\DATA$ converges to
tolerance $\tau=\omega\varepsilon_k$ for every $k\ge0$
in a finite number of steps. Moreover, the number of iterations of $\GALERKIN$ is independent of $k$
due to Proposition \ref{P:cost-galerkin} (computational cost of $\GALERKIN$), whence we deduce
that each loop of $\AFEM$ requires finite
iterations. Thus, the output $u_{k+1}$ satisfies
%
\[
\enorm{u -u_{k+1}} \leq \enorm{ u - \widehat{u}_k} + \enorm{ \widehat{u}_k -u_{k+1}} \le
\big( C_D + C_G \big) \varepsilon_k \quad\forall \, k \geq 0 \,,
\]
%
according to \eqref{E:error-DATA} with $\tau\le\varepsilon_k$ and \eqref{E:output-galerkin}.
Finally, $\AFEM$ terminates after $K$
loops, where $K$ satisfies $\frac{1}{2}\tol < \varepsilon_{K}  \leq \tol$, and the
asserted estimate holds with $C_* = C_D + C_G$.
\end{proof}

This elementary proof gives no insight whether the energy error decays optimally in terms of degrees of freedom.
We assess this fundamental question in Sections \ref{S:conv-rates-coercive} and \ref{S:data-approx},
but investigate it now computationally.
%
\todo{Should we include some insightful numerical experiments, such as Kellogg's example?}


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

\def\gnuplot@output@ps{ps} % required for comparison in \gprawimage

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {html}
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {pdf}

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \edef\gnuplot@output@mode{\csname gnuplot@select@driver@\pgfsysdriver\endcsname}
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

\ifcsname PackageWarning\endcsname
  \let\gnuplot@packagewarning\PackageWarning
\else
  \def\gnuplot@packagewarning#1#2{\immediate\write-1{Package #1 Warning: #2}}
\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
  \gnuplot@packagewarning{gnuplot-lua-tikz}{%
    \noexpand\gp@rawimage is not implemented for \gnuplot@output@mode\space output.%
  }%
}

% Select \gp@rawimage depending on the output mode
\expandafter\let\expandafter\gp@rawimage\csname gp@rawimage@\gnuplot@output@mode\endcsname

\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{%
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext{%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
  \else
    \ifx\gnuplot@output@mode\gnuplot@output@ps
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}%
    \fi
  \fi
}

%
% gnuplottex compatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
% 3-parameter variant gp3point passes style options as well as point type and coordinates
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}
\def\gp3point#1#2#3{%
  \path[solid#2] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#3};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}%
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }%
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex,line width=0pt}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex,line width=0pt}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex,line width=0pt}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds,fit}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode

\endinput


==> notations.tex <==
%------------------------------------------------------------------
\subsection{Function Spaces}
%------------------------------------------------------------------

\begin{tabular}{ll}
  $W^{s}_p(\Omega)$ & Sobolev Space with differentiability $s$ and integrability $p$\\
  $H^s(\Omega)$ & Sobolev Space with differentiability $s$ and integrability $2$ \\
  ${\mathbb S}^{n,0}_\grid$ & Space of continuous piecewise polynomials of degree $\le n$
  over $\grid$ \\
  ${\mathbb S}^{n,-1}_\grid$ & Space of discontinuous piecewise polynomials of degree $\le n$
  over $\grid$ \\
  $\V_\grid$ & Finite element subspace of $H^1_0(\Omega)$ \\
  $\P_n(T)$ & Space of polynomials of degree $\le n$ over $T$ \\
  $\disfct(\grid)$ & $H^{-1}(\Omega)$ - discrete functionals associated with the grid $\grid$ \\
  $\V^+(\grid)$ & Space of test functions for projection operator $P_\grid$
\end{tabular}

%------------------------------------------------------------------
\subsection{Meshes}
%------------------------------------------------------------------

\begin{tabular}{ll}
  $\grid$ & Mesh \\
  $\grid^0$ & Initial mesh \\
  $\grids$ & Collection of all grids $\grid$ emanating from $\grid^0$ \\
  $\marked$ & Marked set \\
  $\vertices =\vertices_\grid$ &Vertices of $\grid$ \\
  $\nodes = \nodes_\grid$ & Nodes of $\grid$ \\
  $\faces = \faces_\grid$ & Faces of $\grid$ \\
  $T$ & Element of $\grid$\\
  $g(T)$ & Generation of element $T$ \\
\end{tabular}


%------------------------------------------------------------------
\subsection{Operators}
%------------------------------------------------------------------

\begin{tabular}{ll}
$I_\grid$ & Lagrange or quasi-interpolation operator over the mesh $\grid$ \\
$P_\grid$ & Projector operator onto discrete data over $\grid$ \\
$E_F$ & Extension operator from face $F$ to discrete neighborhood $\omega_F=\supp\phi_F$
\end{tabular}  

%------------------------------------------------------------------
\subsection{Functions}
%------------------------------------------------------------------

\begin{tabular}{ll}
  $u$ & Solution of the PDE \\
  $\data = (A,c,f)$ & Data \\ 
  $\hdata = (\hA,\hc,\hf)$ & Approximate Data\\
  $\{\phi_z\}_{z\in\vertices}$ & Basis of $C^0$ piecewise linear functions over $\grid$ (partition of unity) \\
  $\phi_T$ & Bubble function over element $T\in\grid$ \\
  $\phi_E$ & Bubble function associated with face $F \in \faces$
\end{tabular} 


%------------------------------------------------------------------
\subsection{Constants}
%------------------------------------------------------------------

\begin{tabular}{ll}
  $C_P$ & Poincar\'e constant \\
  $C_F$ & Friedrichs constant \\
  $\Lambda_0$ & Complexity bisection constant
\end{tabular}
 
%------------------------------------------------------------------
\subsection{Modules}
%------------------------------------------------------------------

\begin{tabular}{ll}
$\AFEM$ &  Algorithm consisting on $\DATA$ and $\GALERKIN$ \\
$\GALERKIN$ & Procedure that iterates $\SOLVE, \ESTIMATE, \MARK, \REFINE$ \\
$\DATA$ &  Procedure than approximates the data $\data$ \\
$\SOLVE$ & Procedure that computes the exact Galerkin solution \\ 
$\ESTIMATE$ & Procedure that computes the estimator $\estG$ \\
$\MARK$ &  Procedure that mark elements $\marked$ of $\mesh$ for refinement \\
$\REFINE$  & Procedure that refines $\marked$ and keeps the mesh conforming \\
$\PROJECT$ & Procedure that computes local data approximation \\
$\ESTIMATEDATA$ & Procedure that  determines local data error estimators \\
$\MARKDATA$ & Procedure that applies a greedy algorithm to mark for data
\end{tabular}


%------------------------------------------------------------------
\subsection{Error Estimators}
%------------------------------------------------------------------

\begin{tabular}{ll}
  $\est_\grid(u_\grid,f)$ & Full error estimator \\
  $\eta_\grid (u_\grid)$ & PDE error estimator \\
  $\zeta_\grid (u_\grid)$ & Quasi error \\
  $\osc_\grid(\data)$ & Data error estimator \\
  $\osc_\grid(A)$ & Diffusion error estimator \\
  $\osc_\grid(c)$ & Reaction error estimator \\
  $\osc_\grid(f)$ & Load error estimator \\
  $\osc_\grid(\data,T)$ & Element data error estimator \\
  $\osc_\grid(A,T)$ & Element diffusion error estimator \\
  $\osc_\grid(c,T)$ & Element reaction error estimator \\
  $\osc_\grid(f,T)$ & Element load error estimator \\
\end{tabular}


==> tools_old.tex <==
\todo{Introduction to be adjusted at the end}
%
We devote this section to discussing basic concepts about
piecewise polynomial approximation in
Sobolev spaces over graded meshes in any dimension $d$. 
We start with the definition of Sobolev number in 
\S \ref{S:sobolev-number} and its role in Sobolev embeddings.

We explore the geometric aspects of mesh refinement for conforming
meshes in \S \ref{S:bisection} and nonconforming meshes in \S
\ref{S:nonconforming-meshes}, but postpone a full discussion until
\S \ref{S:mesh-refinement}. We include a statement about
complexity of the refinement procedure, which turns out to be
instrumental later and will proved in \S \ref{S:mesh-refinement}.

We briefly discuss the construction of finite element spaces in
\S \ref{S:fe-spaces}, along with polynomial interpolation of functions
in Sobolev spaces in \S \ref{S:pol-interp}. This provides local estimates
adequate for comparison of quasi-uniform and graded meshes for $d>1$. We
exploit them in developing the so-called error equidistribution
principle and the construction of suitably graded meshes via
a greedy algorithm in \S \ref{S:constructive}. We conclude that graded
meshes can deliver optimal interpolation rates for certain classes of
singular functions, and thus supersede quasi-uniform refinement.

%-------------------------------------------------------------------------------------
\subsection{\bf The Galerkin Method: Best Approximation}\label{S:Galerkin}
%-------------------------------------------------------------------------------------
%
In order to render the variational problem \eqref{var-prob-general} computable, we let
$\V_N\subset\V$ and $\W_N\subset\W$ be subspaces with the same dimension $N<\infty$ and
consider the Petrov-Galerkin approximation:
%
\begin{equation}\label{E:Galerkin}
u_N \in \V_N: \quad
\bilin{u_N}{w} = \dual{f}{w} \quad\forall \, w \in \W_N.
\end{equation}
%
If $\V_N=\W_N$ this is called Galerkin approximation. Since \eqref{E:Galerkin} is a square algebraic
system, existence and uniqueness of $u_N\in\V_N$ is equivalent to the kernel of the corresponding
linear discrete operator to be trivial. This leads to the following equivalent conditions for unique
solvability \cite[Proposition 1]{NoSiVe:09}.

\begin{lemma}[discrete inf-sup]\label{L:inf-sup_N}
{\it  The following statements are equivalent:
  \begin{enumerate} %[\upshape(1)]
  \setlength{\itemindent}{-0.6em}  
  \item[1.]  %\label{nsv-non-zero_N}
  for every $0\ne v\in\VN$ there exists $w\in\WN$ such that
    $\bilin{v}{w} \ne 0$;
\item[2.] %\label{nsv-inf-sup_N5}
    for every $0\ne w\in\WN$ there exists $v\in\VN$ such that
        $\bilin{v}{w} \ne 0$;
 \item[3.] %\label{nsv-inf-sup_N1}
 the following discrete inf-sup condition holds with a constant $\beta_N>0$
 \begin{equation}\label{E:discrete-inf-sup}
  \infimum_{v\in\VN}\sup_{w\in\WN}\frac{\bilin{v}{w}}{\|v\|_\V \|w\|_\W}
  =
  \infimum_{w\in\WN}\sup_{v\in\VN}\frac{\bilin{v}{w}}{\|v\|_\V \|w\|_\W}
  = \beta_N;
\end{equation}
\item[4.] %\label{nsv-inf-sup_N2}
    \begin{math}
      \displaystyle
      \infimum_{v\in\VN}\sup_{w\in\WN}\frac{\bilin{v}{w}}{\|v\|_\V \|w\|_\W}>0;
    \end{math}
  \item[5.] %\label{nsv-inf-sup_N3}
    \begin{math}
      \displaystyle
      \infimum_{w\in\WN}\sup_{v\in\VN}\frac{\bilin{v}{w}}{\|v\|_\V \|w\|_\W}>0.
    \end{math}
  \end{enumerate}
 } 
\end{lemma}

This is a discrete version of Theorem \ref{T:ex1-var-prob} (Ne\v cas) and leads to the stability bound
%
\begin{equation}\label{E:discrete-stability}
\|u_N\|_{\V} \leq \frac{1}{\beta_N} \|f\|_{\W^*}.
\end{equation}
%
Therefore, $\beta_N^{-1}$ acts as a stability constant for \eqref{E:Galerkin} and is thus 
desirable that it is uniformly bounded below away from zero. This is always the case for
{\it coercive} problems because \eqref{nsv-coercivity} is inherited within the subspaces
$\VN=\WN\subset\V$, whence $\beta_N\ge\alpha>0$. In contrast, a uniform lower bound for {\it saddle point} problems
%
\begin{equation}\label{E:uniform-inf-sup}
\beta_N \ge \beta >0,
\end{equation}
%
requires compatibility between the subspaces $\VN$ and $\WN$ \cite{BoffiBrezziFortin:13}. We will 
come back to this issue in Section \ref{S:conv-rates-infsup}.

If we now subtract \eqref{E:Galerkin} from \eqref{var-prob-general}, we obtain {\it Galerkin orthogonality}
%
\begin{equation}\label{E:Galerkin-orthogonality}
\bilin{u-u_N}{w} = 0 \quad\forall \, w\in\WN.
\end{equation}
%
This relation is instrumental to derive the following best approximation property as
well to develop a posteriori error estimates in Section \ref{S:aposteriori}.

\begin{proposition}[Quasi-Best-Approximation Property]\label{P:QBAP}
  Let $\B\colon\V\times\V\to\R$ be continuous and satisfy
  \eqref{E:discrete-inf-sup}.  Then the error $u-\uN$ satisfies the bound
  \begin{equation}\label{E:best-approximation}
    \|u-\uN\|_\V \leq \frac{\|\B\|}{\beta_N} \min_{v\in\VN} \|u-v\|_\V.
  \end{equation}
\end{proposition}

\begin{proof}
We give a simplified proof, which follows Babu{\v s}ka
\cite{Babuska:71,BabuskaAziz:72} and yields the constant 
$1+\frac{\|\B\|}{\beta_N}$. The asserted constant is due to Xu and Zikatanov
\cite{XuZikatanov:03}.

Combining \eqref{E:discrete-inf-sup}, \eqref{E:Galerkin-orthogonality}, and the
continuity of $\B$, we derive for all $v\in\V_N$
\[
 \beta_N\|u_N-v\|_\V
 \le
 \sup_{w\in\W_N}\frac{\bilin{u_N-v}{w}}{\|w\|_\W}
 =
 \sup_{W\in\W_N}\frac{\bilin{u-v}{w}}{\|w\|_\W}
 \le
 \|\B\| \|u-v\|_\V,
\]	
whence
\[
 \|u_N-v\|_\V\le\frac{\|\B\|}{\beta_N}\|u-v\|_\V.
\]
Using the triangle inequality yields
\[
 \|u-u_N\|_\V\le\|u-v\|_\V+\|v-u_N\|_\V
 \le
 \bigg(1+\frac{\|\B\|}{\beta_N}\bigg)\|u-v\|_\V
\]
for all $v\in\V_N$. It just remains to minimize in $\V_N$.
\end{proof}

The significance of \eqref{E:best-approximation} is that we need to construct discrete spaces
$\VN$ with good approximation properties. We introduce next piecewise polynomial
approximation, which yield the finite element method.

%-------------------------------------------------------------------------------------
\subsection{\bf Finite Element Spaces}\label{S:fe-spaces}
%-------------------------------------------------------------------------------------
%
In this section we focus on the construction of the discrete spaces $\VN$ and $\WN$.
We consider the bilinear forms $\mathcal{B}$ introduced in Section \ref{S:bvp} with emphasis on
the diffusion-reaction case \eqref{bilinear-coercive}. We assume that $\Omega$ is a
bounded Lipschitz domain $\Omega\subset\R^d$ and is partition into a conforming mesh $\grid$
made of simplices $T$ which are assumed to be closed. The intersection of simplices is
a simplex or lower dimension (edge-to-edge triangulation) and
%
\[
\overline{\Omega} = \cup \{T: T\in\grid\}.
\]
%
We will discuss the construction of conforming meshes in Section \ref{S:bisection} by the bisection
method and that of non-conforming meshes in Section \ref{S:nonconforming-meshes}, both for $d=2$.
We will embark on a thorough discussion in Section \ref{S:mesh-refinement}. We assume for the moment 
that $\grid$
is an element of a (possibly infinite) class $\grids$ of {\it shape regular} meshes. To define this
geometric concept, we denote by $\overline{h}_T$ the diameter of $T\in\grid$, by $\underline{h}_T$
the diameter of the largest ball contained in $T$, and impose the restriction
%
\begin{equation}\label{E:shape-regularity}
    \sigma = \sup_{\grid\in\grids} \sup_{T\in\grid} \frac{\overline{h}_T}{\underline{h}_T} < \infty.
\end{equation}
%
Consequently, elements $T$ are not allowed to become asymptotically thin.
 
Given a conforming and shape regular mesh $\grid\in\grids$ we define the finite element space of
continuous piecewise polynomials of degree $n\ge1$
%
\[
{\mathbb S}^{n,0}_\grid := \{v\in C^0(\overline{\Omega})| 
~~v|_T \in \P_n(T) ~~\forall T\in\grid\};
\]
%
note that ${\mathbb S}^{n,0}_\grid\subset H^1(\Omega)$ which makes it adequate for 
\eqref{weak-form}-\eqref{bilinear-coercive}.  We refer to
Braess \cite{Braess:07}, Brenner-Scott \cite{BrennerScott:08}, Ciarlet
\cite{Ciarlet:02} and Siebert \cite{Siebert:12} for a discussion on
the local construction of this space (i.e. Lagrange elements of degree $n\ge1$)
along with its properties.

We focus on the piecewise linear case $n=1$ (Courant
elements), but most results extend to $n>1$. In this vein, global continuity can be simply enforced by imposing continuity at the set $\nodes$ of vertices $z$ of $\grid$, the so-called {\it nodal
values}.

However, the following local construction leads to global continuity.
If $T$ is a generic simplex
of $\grid$, namely the convex hull of $\{z_i\}_{i=0}^d$,
then we associate to each vertex $z_i$ a {\it barycentric
coordinate} $\lambda_i^T$, which is the linear function in $T$ with nodal
value $1$ at $z_i$ and $0$ at the other vertices of $T$. Upon pasting
together the barycentric coordinates $\lambda_z^T$ of all simplices $T$
containing vertex $z\in\nodes$, we obtain a continuous piecewise
linear function $\phi_z\in{\mathbb S}^{1,0}_\grid$ 
as depicted in Figure \ref{nv-F:basis} for $d=2$:
%
\todo{CC: the picture of the star on the right should be coherent with the star seen on the left: as a minimum, a pentagon.}
\begin{figure}[h]
\begin{center}
\includegraphics{figs/fem/pic-2-2}
\hskip2.cm
\includegraphics{figs/fem/pic-2-3}
\end{center}
\caption{Piecewise linear basis function $\phi_z$ corresponding to
  interior node $z$, support $\omega_z$ of $\phi_z$ and scheleton $\gamma_z$,
  the latter being composed of all sides within the interior of
  $\omega_z$.}
\label{nv-F:basis}
\end{figure}
%
The set $\{\phi_z\}_{z\in\nodes}$ of all such functions
is the nodal basis of ${\mathbb S}^{1,0}_\grid$, or Courant basis.
We denote by $\omega_z := \supp (\phi_z)$ the support of
$\phi_z$, from now on called {\it star} associated to $z$, and by
$\gamma_z$ the scheleton of $\omega_z$, namely all the sides
containing $z$.

In view of the definition of $\phi_z$,
we have the following unique representation of any function
$v\in{\mathbb S}^{n,0}(\grid)$
%
\[
v(x) = \sum_{z\in\nodes} v(z) \phi_z(x).
\]
%
The functions $\phi_z$ are non-negative and satisfy the {\it partition of unity} property
%
\begin{equation}
    \sum_{z\in\nodes} \phi_z(x) = 1 \quad\forall \, x\in \Omega.
\end{equation}
%
If we further impose $v(z)=0$ for all $z\in\partial\Omega\cap\nodes$,
then $v\in H^1_0(\Omega)$. We denote by
%
\[
\V_\grid := {\mathbb S}^{n,0}_\grid \cap H^1_0(\Omega)
\]
%
the subspace of finite element functions which vanish on
$\partial\Omega$. Note that we do not explicitly refer to the
polynomial degree, which will be clear in each context.

For each simplex $T\in\grid$, generated by vertices $\{z_i\}_{i=0}^d$,
the {\it dual functions} $\{\lambda_i^*\}_{i=0}^d\subset\P_1(T)$ to the
barycentric coordinates $\{\lambda_i\}_{i=0}^d$ satisfy the
bi-orthogonality relation $\int_T \lambda_i^*\lambda_j=\delta_{ij}$,
and are given by
%
\[
\lambda_i^* = \frac{(1+d)^2}{|T|} \lambda_i - \frac{1+d}{|T|}
\sum_{j\ne i} \lambda_j
\qquad\forall ~0\le i \le d.
\]
%
The {\it Courant dual basis} $\phi_z^*\in{\mathbb S}^{n,-1}(\grid)$ are the 
discontinuous piecewise linear functions over $\grid$ given by
%
\[
\phi_z^* = \frac{1}{\nu_z} \sum_{T\ni z} (\lambda_z^T)^* \chi_T
\qquad\forall ~z\in\nodes,
\]
%
where $\nu_z\in\N$ is the valence of $z$ (number of elements of
$\grid$ containing $z$) and $\chi_T$ is the characteristic function of
$T$. These functions have the same support $\omega_z$ as the nodal
basis $\phi_z$ and satisfy the global bi-orthogonality relation
%
\[
\int_\Omega \phi_z^* \phi_y = \delta_{zy}
\qquad\forall ~z,y\in\nodes.
\]
%

%-------------------------------------------------------------------------------------
\subsection{\bf Polynomial Interpolation in Sobolev Spaces}\label{S:pol-interp}
%-------------------------------------------------------------------------------------
%
If $v\in C^0(\overline{\Omega})$ we define the {\it Lagrange
  interpolant} $I_\grid v$ of $v$ as follows:
%
\[
I_\grid v(x) = \sum_{z\in\nodes} v(z) \phi_z(x),
\]
%
and note that $I_\grid v = v$ for all $v\in {\mathbb S}^{n,0}_\grid$ (i.e. $I_\grid$ is invariant
in ${\mathbb S}^{n,0}_\grid$).
For functions without point values, such as functions in $H^1(\Omega)$
for $d>1$, we need to determine nodal values by averaging. 
For any conforming mesh $\grid\in\grids$,
the averaging process extends beyond nodes and so gives rise to the
discrete neigborhood
%
\begin{displaymath}
  \neighG(\elm)\definedas\{\elm'\in\grid\mid \elm'\cap\elm\neq\emptyset\}
\end{displaymath}
for each element $\elm\in\grid$ along
with the {\it local quasi-uniformity} properties
%
\begin{equation*}
  \max_{\elm\in\grid}
  \#\neighG(\elm) 
  \leq C(\sigma),
  \qquad
  \max_{\elm'\in \neighG(\elm)}
  \frac{\vol{\elm}}{\vol{\elm'}} \leq C(\sigma),
\end{equation*}
where $\sigma$ is the shape regularity coefficient defined in \eqref{E:shape-regularity}.

We introduce now one such operator $I_\grid$ due to Scott-Zhang
\cite{BrennerScott:08,ScottZhang:90}, from now on called {\it
  quasi-interpolation operator}. We focus on polynomial degree $n=1$,
but the construction is valid for any $n$; see
\cite{BrennerScott:08,ScottZhang:90} for details.  We recall that
$\{\phi_z\}_{z\in\nodes}$ is the global Lagrange basis of ${\mathbb
  S}^{1,0}_\grid$, $\{\phi_z^*\}_{z\in\nodes}$ is the global dual
basis, and $\supp\phi_z^*=\supp\phi_z$ for all $z\in\nodes$.  We thus
define $I_\grid: L^1(\Omega) \to {\mathbb S}^{1,0}_\grid$ to be
%
\begin{equation}\label{E:quasi-interpolant}
I_\grid v := \sum_{z\in\nodes} \dual{v}{\phi_z^*} \phi_z,
\end{equation}
%
If $0 \le s \le 2$ is a regularity index and
$1\le p\le\infty$ is an integrability index, then
we would like to prove the {\it quasi-local error estimate}
%
\begin{equation}
\label{E:quasi-interp-error}
 \|D^t(v-I_\grid v)\|_{L^q(\elm)}
 \lesssim
 \helm^{\sob(W^s_p)-\sob(W^t_q)}\|D^s v\|_{L^p(\neighG(\elm))}
\end{equation}
%
for all $T\in\grid$,
provided $0\le t\le s$, $1\leq q \leq\infty$ are such that
$\sob(W^s_p) > \sob(W^t_q)$.

We first recall that $I_\grid$ is invariant in
${\mathbb S}^{1,0}_\grid$, namely,
%
\[
 I_\grid w=w \quad \fa w\in {\mathbb S}^{1,0}_\grid.
\]
%
Since the averaging process giving rise to the values of
$I_\grid v$ for each element $\elm\in\grid$ takes place in the
neighborhood $N_\grid(\elm)$, we also deduce the local
invariance
%
\[
 I_\grid w|_\elm = w \quad \fa w\in \P_1(N_\grid(T))
\]
%
as well as the local stability estimate for any $1\le q \le \infty$
%
\[
\|I_\grid v\|_{L^q(\elm)} \Cleq \|v\|_{L^q(N_\grid(\elm))}.
\]
%
We thus may write
\[
 v - I_\grid v|_\elm
 =
 (v-w) - I_\grid (v-w)|_\elm
\quad\fa \elm\in\grid,
\]
where $w\in\P_{s-1}$ is arbitrary ($w=0$ if $s=0$).  
It suffices now to prove \eqref{E:quasi-interp-error} in the
reference element $\refelm$ and scale back and forth to $T$; 
the definition \eqref{nv-sobolev-number} of Sobolev
number accounts precisely for this scaling. 
We keep the notation $\elm$ for $\refelm$,
apply the inverse estimate for linear polynomials
%
$
 \|D^t(I_\grid v)\|_{L^q(\elm)}
 \lesssim
 \|I_\grid v\|_{L^q(\elm)}
$
%
to $v-w$ instead of $v$, and use the above local stability
estimate, to infer that
%
\[
 \|D^t(v-I_\grid v)\|_{L^q(\elm)}
 \lesssim
 \|v-w\|_{W^t_q(\neighG(\elm))}
 \lesssim
 \|v-w\|_{W^s_p(\neighG(\elm))}.
\]
%
The last inequality is a consequence 
$W^s_p(N_\grid(T)) \subset W^t_q(N_\grid(T))$ because
$\sob(W^s_p) > \sob(W^t_q)$ and $t\leq s$.
Estimate \eqref{E:quasi-interp-error} now follows from the
Bramble-Hilbert lemma \cite[Lemma 4.3.8]{BrennerScott:08}, 
\cite[Theorem 3.1.1]{Ciarlet:02}
\begin{equation}
\label{E:local-BrambleHilbert}
 \inf_{w\in\P_{s-1}(\neighG(\elm))} \| v-P \|_{W^s_p(\neighG(\elm))}
 \lesssim
 \|D^s v\|_{L^p(\neighG(\elm))}.
\end{equation}
%
This proves \eqref{E:quasi-interp-error} for $n=1$. The construction
of $I_\grid$ and ensuing estimate \eqref{E:quasi-interp-error} are still valid
for any $n>1$ \cite{BrennerScott:08,ScottZhang:90}.

\begin{proposition}[quasi-interpolant without boundary values]
\label{P:quasi-interp}
{\it Let $s,t$ be regularity indices with $0\leq t \le s\leq n+1$, and
$1\le p,q\le\infty$  be integrability indices so that
$\sob(W^s_p) > \sob(W^t_q)$.
%
Then there exists a quasi-interpolation operator 
$I_\grid: L^1(\Omega)\to {\mathbb S}^{n,0}_\grid$, which is
invariant in ${\mathbb S}^{n,0}_\grid$ and satisfies
%
\begin{equation}
\label{E:quasi-interp-error-bis}
 \|D^t(v-I_\grid v)\|_{L^q(\elm)}
 \lesssim
 \helm^{\sob(W^s_p)-\sob(W^t_q)}\|D^s v\|_{L^p(\neighG(\elm))}
 \quad\forall T\in\grid.
\end{equation}
% 
The hidden constant in \eqref{E:quasi-interp-error}
depends on the shape coefficient of $\gridk[0]$ and $d$.
}
\end{proposition}

To impose a vanishing trace on $I_\grid v$ we may suitably modify
the averaging process for boundary nodes.
We thus define a set of dual functions with respect 
to an $L^2$-scalar product over ${(d-1)}$-subsimplices contained on 
$\partial\Omega$; see again \cite{BrennerScott:08,ScottZhang:90} 
for details. This retains the invariance
property of $I_\grid$ on ${\mathbb S}^{n,0}(\grid)$ and guarantees that
$I_\grid v$ has a zero trace if $v\in W^1_1(\Omega)$ does.
Hence, the above argument applies and
\eqref{E:quasi-interp-error-bis} follows provided $s\geq1$.

\begin{proposition}[quasi-interpolant with boundary values]
\label{P:quasi-interp-bc}
{\it Let $s,t,p,q$ be as in Proposition \ref{P:quasi-interp}.
There exists a quasi-interpolation operator 
$I_\grid: W^1_1(\Omega)\to {\mathbb S}^{n,0}_\grid$ 
invariant in ${\mathbb S}^{n,0}_\grid$ which
satisfies \eqref{E:quasi-interp-error-bis} for
$s\ge1$ and preserves the boundary values of $v$ provided they are piecewise
polynomial of degree $\le n$. In particular, if $v\in W^1_1(\Omega)$ has a
vanishing trace on $\partial\Omega$, then so does $I_\grid v$.
}
\end{proposition}
%

\begin{remark}[fractional regularity]\label{nv-R:fractional}
  We observe that \eqref{E:quasi-interp-error} does not require the
  regularity indices $t$ and $s$ to be integer.  The proof follows along the
  same lines but replaces the polynomial degree $s-1$ by the greatest
  integer smaller than $s$; the generalization of
  \eqref{E:local-BrambleHilbert} can be taken from
  \cite{DupontScott:80}.
\end{remark}

\begin{remark}[local error estimate for Lagrange interpolant]\label{nv-R:lagrange}
Let the regularity index $s$ and integrability index $1\le p\le \infty$ satisfy
$s-d/p>0$. This implies that 
$\sob(W^s_p)>\sob(L^\infty)$, whence
$W^s_p(\Omega)\subset C(\overline{\Omega})$ and
the Lagrange interpolation operator 
$I_\grid: W^s_p(\Omega)\to {\mathbb S}^{n,0}_\grid$ is well defined and
satisfies the {\it local error estimate}
%
\begin{equation}\label{E:error-lagrange}
 \|D^t(v-I_\grid v)\|_{L^q(\elm)}
 \lesssim
 \helm^{\sob(W^s_p)-\sob(W^t_q)}\|D^s v\|_{L^p(\elm)},
\end{equation}
%
provided $0\le t\le s$, $1\leq q \leq\infty$ are such that
$\sob(W^s_p)>\sob(W^t_q)$.
We point out that $\neighG(\elm)$ in \eqref{E:quasi-interp-error} is
now replaced by $\elm$ in \eqref{E:error-lagrange}. We also remark
that if $v$ vanishes on $\partial\Omega$ so does $I_\grid v$. The
proof of \eqref{E:error-lagrange} proceeds along the same lines as
that of Proposition \ref{P:quasi-interp} except that the nodal
evaluation does not extend beyond the element $\elm\in\grid$
and the inverse and stability estimates over the reference element
are replaced by
%
\[
\|D^t I_\grid v\|_{L^q(\refelm)} \Cleq \|I_\grid v\|_{L^q(\refelm)}
\Cleq \|v\|_{L^\infty(\refelm)}
\Cleq \|v\|_{W^s_p(\refelm)}.
\]
%
\end{remark}

We are now in a position to derive a global interpolation error
estimate.  To this end, it is convenient to introduce the mesh-size
function $h\in L^\infty(\Omega)$ given by
\begin{equation}
\label{E:mesh-size-fct}
 h_{|\elm} = h_\elm \quad\fa \elm\in\grid.
\end{equation}
Notice that the following estimate encompasses the linear as well as
the nonlinear Sobolev scales.

\begin{theorem}[global interpolation error estimate]\label{T:global-interp}
{\it Let $1 \le s \le n+1$, $t=0,1$, $t<s$, and $1 \le p \le q$ satisfy
$r:=\sob(W^s_p) - \sob(W^t_q) > 0$. If $v\in W^s_p(\Omega)$, then
%
\begin{equation}\label{E:global-interp}
\|h^{-r} D^t(v-I_\grid v)\|_{L^q(\Omega)} \Cleq |v|_{W^s_p(\Omega)}.
\end{equation}
}
%
\end{theorem}
%
\begin{proof}
Use Proposition \ref{P:quasi-interp} along with the elementary
property of series
%
$
\sum_n a_n\le (\sum_n a_n^{p/q})^{q/p}
$
for $0<p/q \le 1$.
\end{proof}
%
\todo[inline]{RHN: I think we will need this Theorem for the approximation of data with
$q=2$, $q=\infty$ and $t=0$. We also needed for the approximation of $u$ in $H^1$, so for
$q=2, t=1$. Do we need it for fractional $t$? This is delicate because we will have to localize 
the fractional seminorm $W^t_q$ alla Faermann.}
%--------------------------------------------------------------------------------
\medskip\noindent
\textbf{Continuous vs Discontinuous Approximation of Gradients.}
The preceding discussion might induce us to believe that when dealing with Sobolev functions
$v\in W^1_p(\Omega)$ without pointvalues, namely $1\le p\le d$, global continuity of the quasi-interpolant
might degrade the approximation quality relative to discontinuous approximations. The following
instrumental result by A. Veeser shows that this is not the case \cite[Theorem 2]{Veeser:2016}.

\begin{proposition}[approximation of gradients]\label{P:cont-vs-discont}
 Let $v\in W^1_p(\Omega)$ for $1\le p\le d$. Let $\grid$ be a conforming
  mesh such that its stars are $(d-1)$-face-connected.
  Then there exists a constant $C(\sigma)$ depending on the
  shape regularity coefficient $\sigma$ of \eqref{E:shape-regularity}, the dimension $d$ and the polynomial
  degree $n\ge1$, such that
  %
  \begin{equation}\label{eq:gradient-approx}
    1 \le \frac{\min_{w\in\mathbb {S}^{n,0}_\grid} \|\nabla (v-w)\|_{L^p(\Omega)}}
    {\min_{w\in\mathbb {S}^{n,-1}_\grid} \|\nabla (v-w)\|_{L^p(\Omega)}}
    \le C(\sigma),
  \end{equation}
  %
  where $\mathbb {S}^{n,-1}_\grid$ stands for the space of discontinuous piecewise polynomials of degree $\le n$ over $\grid$.
\end{proposition}

The left inequality in \eqref{eq:gradient-approx} is obvious because $\mathbb {S}^{n,0}_\grid \subset \mathbb {S}^{n,-1}_\grid$. In contrast, the right inequality is delicate and relies on examining quasi-interpolant \eqref{E:quasi-interpolant} \cite[Theorems 1 and 22]{Veeser:2016}. An important consequence of \eqref{eq:gradient-approx} is the following localized version of \eqref{E:global-interp}: $1< s \le n+1$, $1\le p\le 2$ and
$r = \sob(W^s_p) -\sob(W^1_q) > 0$
%
\begin{equation}\label{eq:localized-interp}
\|\nabla(v-I_\grid v)\|_{L^q(\Omega)} \Cleq  \left( \sum_{T\in\grid} h^{pr}_T \| D^s v\|_{L^p(T)}^p \right)^{\frac{1}{p}},
\end{equation}
%
whence the function $v$ does have to belong globally to $W^s_p(\Omega)$ but rather locally, namely
$v\in W^s_p(T)$ for every $T\in\grid$, to get optimal a priori error estimates. This property
will find several applications later.

%--------------------------------------------------------------------------------
\medskip\noindent
\textbf{Quasi-Uniform Meshes.}
We now apply Theorem \ref{T:global-interp} to {\it quasi-uniform} meshes, 
namely meshes $\grid\in\grids$ for which all its elements are of comparable
size $h$, whence
%
\[
h \approx (\#\grid)^{-1/d}.
\]
%
\begin{corollary}[quasi-uniform meshes]\label{nv-C:quasi-uniform}
 {\it Let $1 < s \le n+1$ and $u\in H^s(\Omega)$. If $\grid\in\grids$ is
quasi-uniform, then
%
\begin{equation}\label{E:quasi-uniform-est}
\|\nabla(v-I_\grid v)\|_{L^2(\Omega)} \Cleq |v|_{H^s(\Omega)} (\#\grid)^{-(s-1)/d}.
\end{equation}
}
%
\end{corollary}
%
\begin{remark}[optimal rate]\label{nv-R:optimal-rate}
If $s=n+1$, and so $v$ has the maximal regularity $v\in
H^{n+1}(\Omega)$,
then we obtain the optimal convergence rate in a linear Sobolev scale \looseness=-1
%
\begin{equation}\label{nv-optimal-rate}
\|\nabla(v-I_\grid v)\|_{L^2(\Omega)} \Cleq |v|_{H^{n+1}(\Omega)} (\#\grid)^{-n/d}.
\end{equation}
%
The order $-n/d$ is just dictated by the polynomial degree $n$ and cannot
be improved upon assuming either higher regularity that $H^{n+1}(\Omega)$ 
or a graded mesh $\grid$.
%
\end{remark}

%------------------------------------------------------------------------------------
\noindent
\textbf{Example} (corner singularity in $2d$).
%
To explore the effect of a geometric singularity on \eqref{E:quasi-uniform-est},
we let $\Omega$ be the L-shaped domain of Figure \ref{nv-F:uniform}
and $v\in H^1(\Omega)$ be
%
\[
u(r,\theta) = r^{\frac23} \sin (2\theta/3) - r^{2}/4.
\]
%
This function $v\in H^1(\Omega)$ exhibits the typical corner
singularity of the solution of $-\Delta v = f$ with suitable Dirichlet
boundary condition: $v\in H^s(\Omega)$ for $s<5/3$.
Table \ref{nv-Ta:rate} displays the best
approximation error for polynomial degree $n=1,2,3$
and the sequence of {\it uniform} refinements depicted in Figure \ref{nv-F:uniform}
in the seminorm $|\cdot|_{H^1(\Omega)}$. This 
gives a {\it lower} bound for the interpolation error in \eqref{E:quasi-uniform-est}.
%
\begin{table}[hbtp]
\begin{minipage}{1.\textwidth}
\begin{center}
{\small
\begin{tabular}{|l|r|r|r|}
\hline
\hfil$h$ & linear $(n=1)$ & quadratic $(n=2)$ & cubic $(n=3)$\\
\hline
1/4   & 1.14 &  9.64  &  9.89     \\
1/8   & 0.74 &  0.67  &  0.67     \\
1/16  & 0.68 &  0.67  &  0.67     \\
1/32  & 0.66 &  0.67  &  0.67     \\
1/64  & 0.66 &  0.67  &  0.67     \\
1/128 & 0.66 &  0.67  &  0.67     \\
\hline	
\end{tabular}
}
\end{center}
\end{minipage}
%
\caption{The asymptotic rate of convergence in term of mesh-size $h$
is about $h^{2/3}$, or equivalently $(\#\grid)^{-1/3}$, irrespective
of the polynomial degree $n$. This provides a lower bound for 
$\|v-I_\grid v\|_{L^2(\Omega)}$ and thus shows that
\eqref{E:quasi-uniform-est} is sharp.}
\label{nv-Ta:rate}
%
\end{table}
%
\begin{figure}[ht]
\label{nv-F:uniform}
\begin{center}
\hfil\includegraphics[width=.20\textwidth]%
{figs/rates/mesh1}
\hfil\includegraphics[width=.20\textwidth]%
{figs//rates/mesh2}
\hfil\includegraphics[width=.20\textwidth]%
{figs/rates//mesh3}
\hfil\includegraphics[width=.20\textwidth]%
{figs//rates/mesh4}
\hfil
\end{center}
\caption{Sequence of consecutive uniform meshes for L-shaped domain
  $\Omega$ created by 2 bisections.}
\end{figure}
%
\todo{RHN: There is a problem with the bounding box. This picture will most likely be replaced anyway.}
%

\todo[inline]{RHN: Should we consider Kellogg's example also to illustrate that uniform refinement
goes nowhere?}

Even though $s$ is fractional,
the error estimate \eqref{E:quasi-uniform-est} is still valid
as stated in Remark \ref{nv-R:fractional}. In fact, for uniform refinement,
\eqref{E:quasi-uniform-est} can
be derived by space interpolation between $H^1(\Omega)$ and
$H^{n+1}(\Omega)$. The asymptotic rate $(\#\grid)^{-1/3}$ reported
in Table \ref{nv-Ta:rate} is consistent with
\eqref{E:quasi-uniform-est} and independent of the polynomial degree
$n$; this shows that \eqref{E:quasi-uniform-est} is sharp.
It is also suboptimal as compared with the optimal rate $(\#\grid)^{-n/2}$
of Remark \ref{nv-R:optimal-rate}.

The question arises whether the rate $(\#\grid)^{-1/3}\approx h^{2/3}$ in Table \ref{nv-Ta:rate}
is just a consequence of uniform refinement or
unavoidable.  It is important to realize that
$v\not\in H^s(\Omega)$ for $s\geq5/3$ and thus
\eqref{E:quasi-uniform-est} is not applicable.  However, the problem is not
that second order derivatives of $v$ do not exist but rather that they
are not square-integrable.  In particular, it is true that $v\in
W^2_p(\Omega)$ if $1\le p < 3/2$.  We therefore may apply Theorem
\ref{T:global-interp} with, e.g., $n=1$, $s=2$, and $p\in[1,3/2)$ and
then ask whether the structure of \eqref{E:global-interp} can be
exploited, e.g., by compensating the local behavior of $D^s u$ with
the local mesh-size $h$.  This
enterprise naturally leads to \emph{graded} meshes adapted to $v$.  


\todo[inline]{This new discussion does not use the meshsize. The minimization process is now discrete.}

%-------------------------------------------------------------------------------------
\bigskip\noindent
\textbf{Principle of Error Equidistribution.}
%-------------------------------------------------------------------------------------
%
We investigate the relation between local interpolation error and regularity for
the design of optimal graded meshes adapted to a given function $v\in H^1(\Omega)$ for $d=2$.
We recall that $W^2_1(\Omega)$ is in the same nonlinear Sobolev scale of
$H^1(\Omega)$ but $W^2_1(\Omega) \subset C^0(\overline{\Omega})$ \cite[Lemma 4.3.4]{BrennerScott:08},
that the Lagrange interpolant $I_\grid v$ is well defined and satisfies
%
\begin{equation}\label{E:local-error}
\|\nabla (v- I_\grid v)\|_{L^2(T)} \le C |v|_{W^2_1(T)} =: e_T(v) \quad\forall \, T\in\grid.
\end{equation}
%
We formulate a discrete minimization problem on the surrogate quantity $\be := (e_T(v)_{T\in\grid}\in\R^N$
with $N=\#\grid$: minimize the square of the total $H^1$-error $E_\grid(v)$
%
\[
E_\grid(v)^2 = \sum_{T\in\grid} e_T(v)^2
\]
%
subject to the constraint
%
\[
\sum_{T\in\grid} e_T(v) = C |v|_{W^2_1(\Omega)}.
\]
%
We idealize the problem upon allowing $e_T(v)$ to attain any nonnegative real value despite that
fact that shape regularity of $\grid$ entails geometric restrictions between adjacent elements.
We next form the Lagrangian
%
\[
{\mathcal L}[\be,\lambda] := \sum_{T\in\grid} e_T(v)^2 - \lambda \left(\sum_{T\in\grid} e_T(v)
- C |v|_{W^2_1(\Omega)} \right),
\]
%
with Lagrange multiplier $\lambda\in\R$. We thus realize that the optimality condition reads
%
\[
e_T(v) = \frac{\lambda}{2} \quad\forall \, T\in\grid
\]
%
or that $e_T(v)$ is constant over $\grid$. We rewrite this insightful conclusion as follows:
%
\begin{equation}\label{E:equidistribution}
\begin{minipage}{0.84\linewidth}
{\em A graded mesh is quasi-optimal if the local error is equidistributed.}
\end{minipage}
\end{equation}
%
This calculation yields
%
\[
E_\grid(v)^2 = \frac{\lambda^2}{4} N,\quad
C |v|_{W^2_1(\Omega)} = \frac{\lambda}{2} N, 
\]
%
whence
%
\begin{equation}\label{E:optimal-rate}
E_\grid(v) = C |v|_{W^2_1(\Omega)} N^{-1/2}
\end{equation}
%
is the optimal decay rate but regularity $w\in W^2_1(\Omega)$.
The principle of error equidistribution \eqref{E:equidistribution} was originally derived by
Babu\v{s}ka and Rheinboldt \cite{BabuskaRheinboldt:78} for $d=1$, and extended to $d=2$ by
Nochetto and Veeser \cite[Section 1.6]{NochettoVeeser:2012}, using an idealized continuous minimization
problem involving a meshsize function. The current formulation is closer to applications and does not
require that the power of $h_T$ be positive in \eqref{E:local-error}.


Several remarks are now in order

\begin{remark}[point singularities]\label{R:point-singularities}
Corner singularities \cite{Grisvard:85} as well as singularities due to
intersecting interfaces \cite{Kellogg:75} are of the form
%
\begin{equation}\label{E:corner-sing}
v(x) \approx r(x)^\gamma,
\quad
0<\gamma<1,
\end{equation}
%
for $d=2$. This implies $v\in W^2_1(\Omega)$ for all $\gamma$ and the decay rate \eqref{E:optimal-rate}
provided $\grid$ equidistributes the $H^1$-error. Babu\v ska et al \cite{BaKePi:79}
and Grisvard \cite{Grisvard:85} designed such meshes for corner singularities using weighted $H^2$-regularity.
The preceding approach is more powerful in that it does not require any characterization
of the singularities but instead $v\in W^2_1(\Omega)$, and applies as well to line discontinuities
for $d=2$. We will come back to this point in Section \ref{S:conv-rates-coercive}.
\end{remark}

\begin{remark}[DeVore diagram]\label{R:devore-diagram}
In the linear Sobolev scale, we measure regularity in $L^2$-based Sobolev spaces $H^s(\Omega)$ and
can thus obtain the convergence rate \eqref{E:quasi-uniform-est}, namely
%
\[
\|\nabla(v-I_\grid v)\|_{L^2(\Omega)} \Cleq |v|_{H^s(\Omega)} (\#\grid)^{-(s-1)/2}
\]
%
for $s < 1+\gamma < 2$ and $v$ satisfying \eqref{E:corner-sing}. In the nonlinear Sobolev
scale $W^s_p(\Omega)$
%
\begin{equation}\label{E:nonlinear-Sobolev-scale}
s = \frac{2}{p}
\end{equation}
%
corresponding to $\sob(W^s_p)=\sob{H^1}=0$, we trade differentiability with integrability:
we gain up to differentiability $s=2$ at the expense of lower integrability $p=1$. This
trade-off is at the heart of the optimal estimate \eqref{E:optimal-rate} and is represented
in the so-called DeVore diagram in Fig. \ref{F:devore-diagram}
%
\begin{figure}[h!]\label{F:devore-diagram}
\caption{}
\end{figure}
%
The scale \eqref{E:nonlinear-Sobolev-scale} is not limited to polynomial degree $n=2$, and
thus to differentiability $s\le 2$. If the polynomial degree is $k\ge2$, then the largest
possible value of $s$ is $s=n+1$, which leads to integrability $p$
%
\begin{equation}\label{E:p<1}
 p = \frac{2}{n+1} < 1.
\end{equation}
%
The corresponding Sobolev space must be replaced by the Besov space $B^{n+1}_{p,p}(\Omega)$.
We will come back to this issue in Section \ref{S:conv-rates-coercive}.
\end{remark}

\begin{remark}[non-energy norms]\label{R:non-energy-norms}
%
Property \eqref{E:equidistribution} applies to norms $W^m_q$ for $0\le m \le n+1$ and
$1\le q \le \infty$. We present it here for $m=1$ and $q=2$ for concreteness, but we will
come back to this matter and develop it further in Section \ref{S:data-approx} for data
approximation.
\end{remark}

\begin{remark}[practical meshes]\label{R:practical-meshes}
In contrast to the case $d=1$, discussed in Section \ref{S:univariate}, a serious obstruction for the
realization of the ideal condition \eqref{E:equidistribution} is the geometric constraints induced by mesh shape
regularity. It is clear from \eqref{E:optimal-rate} that \eqref{E:equidistribution} is sufficient for mesh
optimality. A key question is whether estimates of the form $E_\grid(v) \lesssim N^{-1/2}$ can be achieved
under practical but weaker conditions than \eqref{E:equidistribution}.
In Section \ref{S:bisection} we study the bisection method, a popular technique for
conforming mesh refinement with optimal complexity, and in Section \ref{S:nonconforming-meshes} we extend
its analysis to non-conforming meshes. Moreover, in Section \ref{S:constructive-approximation}
we show that quasi-optimal  bisection meshes that obey \eqref{E:optimal-rate} can be constructed
in practice.
\end{remark}

%-------------------------------------------------------------------------------------
\subsection{\bf Conforming Meshes: The Bisection Method}\label{S:bisection}
%-------------------------------------------------------------------------------------

In order to approximate functions in $W^k_p(\Omega)$ by piecewise
polynomials, we decompose $\Omega$ into simplices. We briefly
discuss the {\em bisection} method, the most elegant and successful technique
for subdividing $\Omega$ in any dimension into a conforming mesh. 
We also discuss briefly 
nonconforming meshes in \S \ref{S:nonconforming-meshes}. 
We present complete proofs, especially of the complexity of bisection, later in 
\S \ref{S:mesh-refinement}. 

We focus on $d=2$ and follow Binev, Dahmen, and DeVore
\cite{BiDaDeV:04}, but the results carry over to any dimension $d>1$
(see Stevenson \cite{Stevenson:08}). We refer to Nochetto, Siebert,
and Veeser \cite{NoSiVe:09} for a rather complete discussion for
$d>1$. \looseness=-1

Let $\grid$ denote a {\it mesh} (triangulation or grid) made of
simplices $T$, and let $\grid$ be {\it conforming} (edge-to-edge). Each
element is labeled, namely it has an edge $E(T)$ assigned for
refinement (and an opposite vertex $v(T)$ for $d=2$); 
see Figure \ref{nv-F:edge-vertex}.

\begin{figure}[ht]
	\centering
	\includegraphics{figs/bisection/pic-3-1}
        \caption{Triangle $T\in\grid$ with vertex $v(T)$ and opposite
          refinement edge $E(T)$. The bisection rule for $d=2$ consists of
          connecting $v(T)$ with the midpoint of $E(T)$, thereby giving rise to
          children $T_1,T_2$ with common vertex $v(T_1)=v(T_2)$, the
          newly created vertex, and 
          opposite refinement edges $E(T_1), E(T_2)$.\label{nv-F:edge-vertex}}
\end{figure}
%
The bisection method consists of a suitable {\it labeling} of the initial mesh
$\grid_0$ and a rule to assign the refinement edge to the two
children. For $d=2$ we consider the {\it newest vertex bisection}
as depicted in Figure \ref{nv-F:edge-vertex}.
For $d>2$ the situation is more complicated and one needs the
concepts of type and vertex order \cite{NoSiVe:09, Stevenson:08}.

Bisection creates a \textit{unique} master
forest $\mathbb{F}$ of binary trees with infinite depth, where each
node is a simplex (triangle in 2d), its two successors are the two
children created by bisection, and the roots of the binary trees are
the elements of the initial conforming partition $\grid_0$. It is
important to realize that, no matter how an element arises in the
subdivision process, its associated newest vertex is unique and only
depends on the labeling of $\grid_0$: so $v(T)$ and $E(T)$ are
independent of the order of the subdivision process for all
$T\in\mathbb{F}$; see Lemma \ref{L:unique-labeling} in 
\S \ref{S:mesh-refinement}.
\todo{Cite this correctly!}
Therefore, $\mathbb{F}$ is unique.

A finite subset $\mathcal{F}\subset\mathbb{F}$ is called a
\textit{forest} if $\grid_0\subset\mathcal{F}$ and the nodes of
$\mathcal{F}$ satisfy
\begin{itemize}
	\item[$\bullet$] all nodes of $\mathcal{F}\setminus\grid_0$ have a predecessor;
	\item[$\bullet$] all nodes in $\mathcal{F}$ have either two successors or none.
\end{itemize}
Any node $T\in\mathcal{F}$ is thus uniquely connected with a node
$T_0$ of the initial triangulation $\grid_0$, i.e. $T$ belongs to the
infinite tree ${\mathbb{F}}(T_0)$ emanating from $T_0$.
Furthermore, any forest may have
\textit{interior nodes}, i.e. nodes with successors, as well as
\textit{leaf nodes}, i.e. nodes without successors. The set of leaves
corresponds to a mesh (or triangulation, grid, partition) 
$\grid=\grid(\mathcal{F})$ of $\grid_0$ which may not
be conforming or edge-to-edge. 

We thus introduce the set  $\grids$ of all conforming refinements of 
$\gridk[0]$:
%
\begin{displaymath}
  \grids := \{\grid = \grid(\mathcal{F}) \mid \mathcal{F}\subset\mathbb{F} 
  \text{ is finite and }\grid(\forest) \text{ is conforming}\}.
\end{displaymath}
%
If $\gridk[*]=\grid(\forest_*)\in\grids$ is a conforming refinement of
$\grid=\grid(\forest)\in\grids$, we write $\gridk[*]\ge\grid$ and understand this
inequality in the sense of trees, namely $\forest\subset\forest_*$.

\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.75]{figs/bisection/pic-3-2}
        \caption{Sequence of bisection meshes $\{\gridk[k]\}_{k=0}^2$ starting
        from the initial mesh $\gridk[0]=\{T_i\}_{i=1}^4$ with longest
        edges labeled for bisection. Mesh
        $\gridk[1]$ is created from $\gridk[0]$ upon bisecting $T_1$
        and $T_4$, whereas mesh $\gridk[2]$ arises from $\gridk[1]$
        upon refining $T_6$ and $T_7$. The bisection rule is described
        in Figure \ref{nv-F:edge-vertex}.\label{nv-F:sequence}}
\end{figure}
%
\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.65]{figs/bisection/pic-3-3}
        \caption{Forest $\forest_2$ corresponding to the grid sequence
          $\{\gridk[k]\}_{k=0}^2$ of Figure \ref{nv-F:sequence}. The
          roots of $\forest_2$ form the initial mesh $\gridk[0]$
          and the leaves of $\forest_2$ constitute the conforming
          bisection mesh $\gridk[2]$. Moreover, each level of
          $\forest_2$ corresponds to all elements with generation 
          equal to the level.\label{nv-F:tree}}
\end{figure}
\medskip\noindent
\textbf{Example:}
Consider $\grid_0=\{T_i\}_{i=1}^4$ and the longest edge
to be the refinement edge. Figure \ref{nv-F:sequence}
displays a sequence of conforming meshes $\gridk[k]\in\grids$
created by bisection.
%

\noindent
Each element $T_i$ of $\grid_0$ is a root of a finite tree
emanating from $T_i$, which together form the forest $\forest_2$
corresponding to mesh $\gridk[2]=\grid(\forest_2)$.
Figure \ref{nv-F:tree} displays $\forest_2$, whose leaf nodes are
the elements of $\gridk[2]$. 

\medskip\noindent
%----------------------------------------------------------------------------
\textbf{Properties of Bisection.}
We now discuss several crucial geometric properties of bisection.
We start with the concept of shape regularity. For any $T\in\grid$,
we define

\begin{minipage}[b]{0.3635\linewidth}
\includegraphics{figs/bisection/pic-1-3}
\end{minipage}
\begin{minipage}[b]{0.6\linewidth}
\begin{align*}
	&\overline{h}_T=\diam(T)\\
	&h_T=|T|^{1/d}\\
	&\underline{h}_T=2\sup\{r>0\,|\, B(x,r)\subset T \text{ for }x\in T\}.
\end{align*}
\vspace{0.35cm}
\end{minipage}
%
Then
%
\[
\underline{h}_T \le h_T \le \overline{h}_T\le \sigma \underline{h}_T
\qquad\forall T\in\grid,
\]
%
where $\sigma>1$ is the shape regularity constant of \eqref{E:shape-regularity}. 
The next lemma guarantees that bisection keeps $\sigma$ bounded.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.9\hsize]{figs/bisection/shape_gen-2d}
  \caption{Bisection produces at most 4 similarity classes for any
    triangle.\label{nv-F:2dsim-gen}}
\end{figure}
%
\begin{lemma}[shape regularity]\label{nv-L:shape-reg}
\it The partitions $\grid$ generated by newest vertex bisection satisfy a
uniform minimal angle condition, or equivalently $\sigma$ is uniformly
bouunded, only depending on the initial partition $\gridk[0]$.
\end{lemma}
%
\begin{proof}
Each $T\in\gridk[0]$ gives rise to a fixed number of similarity
classes, namely $4$ for $d=2$ according to Figure \ref{nv-F:2dsim-gen}.
This, combined with the fact that $\#\gridk[0]$ is finite, yields
the assertion.
\end{proof}

We define the {\it generation (or level)} $g(T)$ of an 
element $T\in\grid$ as the number of bisections needed to create $T$
from its ancestor $T_0\in\gridk[0]$. Since bisection splits an element
into two children with equal measure, we realize that
%
\begin{equation}\label{nv-mesh-gen}
h_T = 2^{-g(T)/2} h_{T_0} \qquad\forall T\in\grid.
\end{equation}
%
Referring to Figure \ref{nv-F:tree} we observe that
the leaf nodes $T_9,T_{10},T_{11},T_{12}$ have generation $2$, whereas
$T_5,T_8$ have generation $1$ and $T_2,T_3$ have generation $0$.

The following geometric property is a simple consequence of
\eqref{nv-mesh-gen}.
%
\begin{lemma}[element size vs generation]\label{nv-L:diam-gen}
\it There exist constants $0<D_1<D_2$, only depending on $\gridk[0]$, such
that
%
\begin{equation}\label{nv-diam-gen}
D_1  2^{-g(T)/2} \le h_T < \overline{h}_T \le D_2  2^{-g(T)/2}
\qquad\forall T\in\grid.
\end{equation}
%
\end{lemma}

%-----------------------------------------------------------------------------------
\medskip\noindent
\textbf{Labeling and Bisection Rule.}
%
Whether the recursive application of bisection does not lead to
inconsistencies depends on a suitable initial labeling of edges and a 
bisection rule. For $d=2$ they are simple to state \cite{BiDaDeV:04},
but for $d>2$ we refer to Condition (b) of Section 4
of \cite{Stevenson:08}.
Given $T\in\grid$ with generation $g(T)=i$, we assign the label $(i+1,i+1,i)$ to $T$ 
with $i$ corresponding to the refinement edge $E(T)$. 
The following rule dictates how the labeling changes with refinement: 
the side $i$ is bisected and both new sides as well as the bisector 
are labeled $i+2$ whereas the remaining labels do not change.
%
To guarantee that the label of an edge is independent of the elements
sharing this edge, we need a special labeling for $\grid_0$ \cite{BiDaDeV:04}: 
%
\begin{equation}\label{nv-initial-label}
\begin{minipage}{0.75\linewidth}
\emph{edges of $\grid_0$ have labels $0$ or $1$ and all elements
  $T\in\grid$ have exactly two edges with label $1$ and one with label
  $0$}.
\end{minipage}
\end{equation}
%
It is not obvious that such a labeling exists, but if it does then all
elements of $\gridk[0]$ can be split into pairs of compatibly
divisible elements.
We refer to Figure \ref{nv-F:labeling} for an example of initial
labeling of $\gridk[0]$ satisfying \eqref{nv-initial-label}
and the way it evolves for two successive
refinements $\gridk[2]\ge\gridk[1]\ge\gridk[0]$ corresponding to
Figure \ref{nv-F:sequence}. 
%
%------------------------------------------------------------------------------
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.75]{figs/bisection/pic-3-4}
        \caption{Initial labeling and its evolution for the sequence
          of conforming refinements
          $\gridk[0]\le\gridk[1]\le\gridk[2]$
          of Figure \ref{nv-F:sequence}. \label{nv-F:labeling}}
\end{figure}


To guarantee \eqref{nv-initial-label} we can proceed as follows:
given a coarse mesh of elements $T$ we can bisect twice each $T$ and
label the $4$ grandchildren, as indicated in Figure
\ref{nv-F:initial-label-2d} 
for the resulting mesh $\grid_0$ to satisfy the initial labeling
\cite{BiDaDeV:04}.
%
\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.8]{figs/bisection/pic-3-5}
        \caption{Bisecting each triangle of $\gridk[0]$ twice and
          labeling edges in such a way that all boundary edges have
          label 1 yields an initial mesh satisfying
          \eqref{nv-initial-label}. \label{nv-F:initial-label-2d}}
\end{figure}
%
A similar, but much trickier, construction can be made in any
dimension $d>2$ (see Stevenson \cite{Stevenson:08}). For $d=3$ the
number of elements increases by an order of magnitude, which indicates
that \eqref{nv-initial-label} is a severe restriction in
practice. Finding alternative, more practical, conditions is an open 
and important problem.
%
\todo[inline]{Is there now an alternative? For quadrilateral meshes with handing nodes
  this is not an issue, and these meshes are easier to handle for $d>2$ Should
  we comment on this here?
}

%----------------------------------------------------------------------------------
\medskip\noindent
\textbf{The Procedure $\REFINE$.}
%
Given $\grid\in\grids$ and a subset $\marked\subset\grid$ of marked
elements, the procedure
%
\[
\gridk[*] = \REFINE (\grid,\marked)
\]
%
creates a new conforming refinement $\gridk[*]$ of $\grid$ by
bisecting all elements of $\marked$ at least once and perhaps
additional elements to keep conformity.

Conformity is a constraint in the refinement procedure that prevents
it from being completely local. The propagation of refinement beyond
the set of marked elements $\marked$ is a rather delicate matter,
which we discuss later in \S \ref{S:mesh-refinement}. For
instance, we show that a naive estimate of the form
%
\[
\#\gridk[*] - \#\grid \le \Lambda_0 ~\#\marked
\]
%
is {\it not} valid with an absolute constant $\Lambda_0$ independent of the
refinement level. This can be repaired upon considering the cumulative
effect for a sequence of conforming bisection meshes
$\{\gridk\}_{k=0}^\infty$.
This is expressed in the following crucial complexity result due to
Binev, Dahmen, and DeVore \cite{BiDaDeV:04} for $d=2$ 
and Stevenson \cite{Stevenson:08} for $d>2$. We present a complete
proof later in \S \ref{S:mesh-refinement}.

\begin{theorem}[complexity of $\REFINE$]\label{nv-T:complexity-refine}
{\it If $\gridk[0]$ satisfies the initial labeling
\eqref{nv-initial-label} for $d=2$, or that in \cite[Section 4]{Stevenson:08}
for $d>2$,
then there exists a constant $\Lambda_0>0$ only depending on
$\gridk[0]$ and $d$ such that for all $k\ge 1$
}
%
\[
\#\gridk - \#\gridk[0] \le \Lambda_0 \sum_{j=0}^{k-1} \# \markedk[j].
\]
%
\end{theorem}
%
If elements $T\in\marked$ are to be bisected $b\ge1$ times, then the
procedure \REFINE can be applied recursively, and 
Theorem \ref{nv-T:complexity-refine} remains valid with $\Lambda_0$
also depending on $b$.

%---------------------------------------------------------------------------------
\subsection{\bf Constructive Approximation}\label{S:constructive-approximation}
%---------------------------------------------------------------------------------
We now construct graded bisection meshes $\grid$ for
$n=1,d=2$ that achieve the optimal
decay rate $(\#\grid)^{-1/2}$ of \eqref{E:optimal-rate}
under the global regularity assumption 
%
\begin{equation}\label{nv-weaker-reg}
	v\in W^2_p(\Omega),\quad p>1.
\end{equation}
%
Therefore, $W^2_p(\Omega)$ is strictly above the Sobolev line $s=p/2$ of \eqref{E:nonlinear-Sobolev-scale}
for $s=2$, whence $W^2_p(\Omega)$ is compactly embedded into $H^1(\Omega)$ according to
Lemma \ref{L:embedding} (Sobolev embedding). This in turn reconciles the principle of error equidistribution \eqref{E:equidistribution} with the geometric constraints due to shape regularity for $d=2$.

Following the work of Binev et al. \cite{BiDaDeVPe:02}, we use a
greedy algorithm that is based on the knowledge of the element
errors and on bisection.
%
The algorithm hinges on \eqref{E:equidistribution}:
if $\delta>0$ is a given tolerance, the element error is
equidistributed, that is $e_T(v)\approx\delta$, and the global error
decays with maximum rate $(\#\grid)^{-1/2}$, then
%
\[
\delta^2 \#\grid
 \approx
 \sum_{T\in\grid} e_T(v)^2
 =
 |v-I_\grid v|^2_{H^1(\Omega)}
 \lesssim
 (\#\grid)^{-1}
\]
%
that is $\#\grid\lesssim\delta^{-1}$. With this in mind, we impose
$e_T(v)\le\delta$ as a threshold to stop refining and expect
$\#\grid\Cleq\delta^{-1}$.
%
The following algorithm implements this idea.

\begin{algo}[Greedy Algorithm] \label{algo:greedy}
Given a
tolerance $\delta>0$ and a conforming mesh $\grid_0$, \textsf{GREEDY} finds
a conforming refinement $\grid\ge\grid_0$ of $\grid_0$ by bisection
such that $e_T(v)\le\delta$ for all $T\in\grid$: let $\grid=\grid_0$
and
%
\begin{algotab}
  \> $\textsf{GREEDY}(\grid,\delta,v)$\\
  \>  while $\marked :=\{T\in\grid\,|\,e_T(v)>\delta\}\ne\emptyset$\\
  \> \> $\grid := \REFINE(\grid,\marked)$\\
  \> end while\\
  \> return($\grid$)
\end{algotab}
%
\end{algo}

Since $W^2_p(\Omega)\subset
C^0(\overline{\Omega})$, because $p>1$, we can use the Lagrange interpolant
and local estimate \eqref{E:error-lagrange} with 
$r=\sob(W^2_p)-\sob(H^1)=2-2/p>0$.
We deduce
%
\begin{equation}\label{E:termination}
	e_T(v)\lesssim h_T^r\,\|D^2 v\|_{L^p(T)}.
\end{equation}

%
The quality of the resulting mesh is assessed next in a slightly more general setting needed later in Section~\ref{S:data-approx} for data approximation. To this end, we follow \cite{bonito2016high} (Proposition~1 and Corollary 1). We consider a generic (possibly vector-valued) function $v:\Omega \subset \mathbb R^d \rightarrow \mathbb R^M$, $M\geq 1$ and denote by $\{ e_T(v) \}_{T \in \grid} \subset \mathbb R^+$ the abstract local errors used in the \textsf{GREEDY} procedure. Rather than \eqref{E:termination}, we assume that
\begin{equation}\label{A:termination_abstract}
e_T(v) \lesssim h_T^r | v |_{p,T}, \qquad r>0, \quad T\in \grid,
\end{equation}
where for $0<p\leq \infty$, $\{ |v|_{p,T}\}_{T\in \grid} \subset \mathbb R$ satisfies  $\left(\sum_{T \in \grid} | v |_{p,T}^p\right)^{1/p} \leq | v |_{p,\Omega}$ (with the usual modification when $p=\infty$) and $|v|_{p,\Omega}$ denotes a quantity only depending on $v$, $\Omega$, and $p$; note that we allow $0<p<1$.

\begin{proposition}[abstract greedy]\label{P:abstract_greedy}
Let $\gridk[0]$ be an initial subdivision satisfying the initial labeling
\eqref{nv-initial-label} for $d=2$, or that in \cite[Section 4]{Stevenson:08}
for $d>2$. Assume that \eqref{A:termination_abstract} holds for some $v:\Omega \subset \mathbb R^d \rightarrow \mathbb R^M$, $M\geq 1$, with $|v|_{p,\Omega} < \infty$.
Then $\textsf{GREEDY}(\grid_0,\delta,v)$ terminates in a finite number of iterations with local errors verifying $e_T(v) < \delta$, $T\in \grid$. Furthermore, the output 
$\grid\in\grids$ of \textsf{GREEDY} satisfies
%
\begin{equation}\label{E:greedy_complexity}
 \#\grid-\#\grid_0\lesssim |\Omega|^{\frac{rp}{d+rp}} \left(\delta^{-1} |v|_{p,\Omega}\right)^\frac{dp}{d+rp}.
\end{equation}
\end{proposition}
\begin{proof}
In view of \eqref{A:termination_abstract}, $h_T$ decreases
monotonically to $0$ with bisection whence \textsf{GREEDY} terminates in finite number $k\ge 1$ of
iterations. Upon termination, the local errors satisfy $e_T(v) < \delta$ by construction. 

Let $\marked=\marked_0\cup\dots\cup\marked_{k-1}$ 
be the set of marked elements. We organize the elements in $\marked$ 
by size in such a way that allows for a counting argument. Let 
${\mathcal P}_j$ be the set of elements $T$ of $\marked$ with size
\[
 2^{-(j+1)}
 \le
 |T|<2^{-j}
\quad\Rightarrow\quad
 2^{-(j+1)/d}\le h_T<2^{-j/d}.
\]
We proceed in several steps.

\step{1} We first observe that all $T$'s in ${\mathcal P}_j$ are
\emph{disjoint}. This is because if $T_1,\,T_2\in {\mathcal P}_j$ and $\mathring{T}_1\cap\mathring{T}_2\neq\emptyset$, then one of them is contained in the other, say $T_1\subset T_2$, due to the bisection procedure \todo{AB: here we need the bisection procedure to be defined for any $d$. RHN: We only have a statement at the beginning of Section \ref{S:bisection}}. 
Thus 
\[
	|T_1|\le\frac{1}{2}\,|T_2|
\]
contradicting the definition of ${\mathcal P}_j$. This implies 
\begin{equation}\label{nv-small}
 2^{-(j+1)}\,\#{\mathcal P}_j
 \le
 |\Omega|
\quad\Rightarrow\quad
 \#{\mathcal P}_j\le|\Omega|\, 2^{j+1}.
\end{equation}
%
\step{2} In light of \eqref{E:termination}, we have for $T\in {\mathcal P}_j$
\[
	\delta\le e_T(v) \lesssim 2^{-(j/d)r}|v|_{p,T}.
\]
Therefore 
\[
\delta^{p}\,\#{\mathcal P}_j\lesssim 2^{-(j/d)rp}
\sum_{T\in{\mathcal P}_j}|v|_{p,T}^p\le 2^{-(j/d)rp}\, |v|_{p,\Omega}^p
\]
whence 
\begin{equation}\label{nv-large}
	\#{\mathcal P}_j\lesssim \delta^{-p}\,2^{-(j/d)rp}\,|v|^p_{p,\Omega}.
\end{equation}
%
\step{3} The two bounds for $\#{\mathcal P}$ in \eqref{nv-small} and
\eqref{nv-large} are complementary. The first is good for $j$ small
whereas the second is suitable for $j$ large (think of $\delta\ll
1$). The crossover takes place for $j_0$ such that 
%
\[
2^{j_0+1}|\Omega| \approx \delta^{-p}\,2^{-j_0(rp/d)}|v|^p_{p,\Omega}
\quad\Rightarrow\quad 
2^{j_0}\approx \left(|\Omega|^{-1} \delta^{-p} |v|_{p,\Omega}^p\right)^{\frac{d}{d+rp}}.
\]
%
\step{4} We now compute 
%
\[
\#\marked=\sum_j\#{\mathcal P}_j\lesssim
\sum_{j\le j_0}2^j|\Omega|+\delta^{-p}\,|v|^p_{p,\Omega}
\sum_{j>j_0}(2^{-rp/2})^j.
\]
%
Since 
%
\[
\sum_{j\le j_0}2^j\approx 2^{j_0},
\qquad \sum_{j>j_0}(2^{-rp/d})^j\lesssim 2^{-(rp/d)j_0}
\]
%
we can write 
%
\[
\#\marked\lesssim |\Omega|^{1-\frac{d}{d+rp}}\big(\delta^{-1} | v |_{p,\Omega}\big)^{\frac{dp}{d+rp}}
\]
%
We finally apply Theorem \ref{nv-T:complexity-refine} (complexity of \REFINE) to arrive at 
%
\[
\#\grid-\#\grid_0\lesssim \#\marked\lesssim |\Omega|^{\frac{rp}{d+rp}} \big(\delta^{-1} | v |_{p,\Omega}\big)^{\frac{dp}{d+rp}}.
\]
%
This concludes the proof.
\end{proof}

Proposition~\ref{P:abstract_greedy} above provides an estimate on the number of elements in the subdivision constructed by \textsf{GREEDY} to reduce the local errors below the tolerance $\delta$, i.e. $\max_{T\in \grid} e_T(v) < \delta$.
The next corollary discusses the accumulation of the local error in $l^q$, $p\leq q < \infty$.
This is motivated by the question of constructing an optimal subdivision for the interpolation error. In this case $e_T(v) = |v-I_\grid v|_{H^1(T)}$ and the global interpolation error is obtained by accumulating the local error in $l^2$, $|v-I_\grid v|_{H^1(\Omega)} = \left(\sum_{T\in \grid} e_T(v)^2\right)^{1/2}$. The case $q \not = 2$ will be needed for the data approximation discussed in Section~\ref{S:data-approx}.

\begin{corollary}[abstract greedy error estimates in $l^q$]\label{C:abstract_greedy}
 Let $\gridk[0]$ be an initial subdivision satisfying the initial labeling
\eqref{nv-initial-label} for $d=2$, or that in \cite[Section 4]{Stevenson:08}
for $d>2$.
Let $0<p\leq q < \infty$. Let $s>1/p-1/q$ and assume that \eqref{A:termination_abstract} holds with $r:=d(s-1/p+1/q)>0$.
 Then for $N > \#\grid_0$ integer, there exits $\grid\in\grids$ such that 
 $$
 \left(\sum_{T \in \grid} e_T(v)^q\right)^{1/q} \lesssim | \Omega|^{r/d}   |v|_{p,\Omega} N^{-s}, \qquad \#\grid - \#\grid_0 \lesssim N.
 $$
 \end{corollary}
%
\begin{proof}
In view of the complexity estimate \eqref{E:greedy_complexity} of \textsf{GREEDY}, we choose
%
\[
\delta = | \Omega|^{r/d} | v|_{p,\Omega} N^{-\frac{d+rp}{dp}}
\]
%
as a target tolerance to readily deduce
%
\[
\#\grid - \#\grid_0 \lesssim N.
\]
%
Furthermore, the subdivision constructed by \textsf{GREEDY} is such that the local errors satisfy $e_T(v) < \delta$ for all $T\in \grid$. 
Therefore, since $\frac{d+rp}{dp} = \frac{1+sq}{q}$, we have
$$
\left(\sum_{T \in \grid} e_T(v)^q\right)^{1/q}  \lesssim \delta (\#\grid)^{1/q} \lesssim | \Omega|^{r/d} | v|_{p,\Omega} N^{-\frac{1+qs}q} N^{1/q} \lesssim  | \Omega|^{r/d} | v|_{p,\Omega} N^{-s}
$$
as desired.
\end{proof}

We are now in position to show that \textsf{GREEDY} constructs optimal graded meshes for the interpolation error in $H^1(\Omega)$ alluded to at the beginning of this section.

\begin{corollary}[optimal convergence rate]\label{C:optimal-mesh}
{\it Let $v\in H^1_0(\Omega)$ \todo{AB: why do you need vanishing boundary conditions here?} satisfy $v \in W^2_p(\Omega)$ for $1<p\leq 2$ and $d=2$. Then \textsf{GREEDY} 
yields graded bisection meshes $\grid$ so that}
%
$$
| v - I_\grid v|_{H^1(\Omega)} \lesssim | \Omega |^{1-1/p} \|D^2 v\|_{L^p(\Omega)} (\#\grid-\#\grid_0)^{-1/2}.
$$
\end{corollary}
%
\begin{proof}
We invoke Corollary~\ref{C:abstract_greedy} with $r=2-2/p$, $q=2$, whence $s=1/2$.
\end{proof}

\todo[inline]{AB: old text commented here}
\begin{comment}
The quality of the resulting mesh is assessed next.
\todo[inline]{This algorithm applies to more general situations. Should we discuss it
  here already in full generality and apply it later for data approximation?}

\begin{theorem}[greedy]\label{T:greedy}
If $v\in H^1_0(\Omega)$ verifies \eqref{nv-weaker-reg}, then \textsf{GREEDY} terminates in finite
number of iterations. The output 
$\grid\in\grids$ of \textsf{GREEDY} satisfies
%
\[
|v-I_\grid v|_{H^1(\Omega)}\le \delta(\#\grid)^{1/2},
\qquad \#\grid-\#\grid_0\lesssim \delta^{-1}\,|\Omega|^{1-1/p}\|D^2 v\|_{L^p(\Omega)}.
\]
\end{theorem}
\begin{proof}
In view of \eqref{E:termination}, $h_T$ decreases
monotonically to $0$ with bisection whence \textsf{GREEDY} terminates in finite number $k\ge 1$ of
iterations. Let $\marked=\marked_0\cup\dots\cup\marked_{k-1}$ 
be the set of marked elements. We organize the elements in $\marked$ 
by size in such a way that allows for a counting argument. Let 
${\mathcal P}_j$ be the set of elements $T$ of $\marked$ with size
\[
 2^{-(j+1)}
 \le
 |T|<2^{-j}
\quad\Rightarrow\quad
 2^{-(j+1)/2}\le h_T<2^{-j/2}.
\]
We proceed in several steps.

\step{1} We first observe that all $T$'s in ${\mathcal P}_j$ are
\emph{disjoint}. This is because if $T_1,\,T_2\in {\mathcal P}_j$ and $\mathring{T}_1\cap\mathring{T}_2\neq\emptyset$, then one of them is contained in the other, say $T_1\subset T_2$, due to the bisection procedure. Thus \[
	|T_1|\le\frac{1}{2}\,|T_2|
\]
contradicting the definition of ${\mathcal P}_j$. This implies 
\begin{equation}\label{nv-small}
 2^{-(j+1)}\,\#{\mathcal P}_j
 \le
 |\Omega|
\quad\Rightarrow\quad
 \#{\mathcal P}_j\le|\Omega|\, 2^{j+1}.
\end{equation}
%
\step{2} In light of \eqref{E:termination}, we have for $T\in {\mathcal P}_j$
\[
	\delta\le e_T(v) \lesssim 2^{-(j/2)r}\|D^2 v\|_{L^p(T)}.
\]
Therefore 
\[
\delta^{p}\,\#{\mathcal P}_j\lesssim 2^{-(j/2)rp}
\sum_{T\in{\mathcal P}_j}\|D^2 v\|^p_{L^p(T)}\le 2^{-(j/2)rp}\,\|D^2 v\|^p_{L^p(\Omega)}
\]
whence 
\begin{equation}\label{nv-large}
	\#{\mathcal P}_j\lesssim \delta^{-p}\,2^{-(j/2)rp}\,\|D^2 v\|^p_{L^p(\Omega)}.
\end{equation}
%
\step{3} The two bounds for $\#{\mathcal P}$ in \eqref{nv-small} and
\eqref{nv-large} are complementary. The first is good for $j$ small
whereas the second is suitable for $j$ large (think of $\delta\ll
1$). The crossover takes place for $j_0$ such that 
%
\[
2^{j_0+1}|\Omega| \approx \delta^{-p}\,2^{-j_0(rp/2)}\|D^2
v\|^p_{L^p(\Omega)}
\quad\Rightarrow\quad 
2^{j_0}\approx \delta^{-1}\,\frac{\|D^2 v\|_{L^p(\Omega)}}{|\Omega|^{1/p}}.
\]
%
\step{4} We now compute 
%
\[
\#\marked=\sum_j\#{\mathcal P}_j\lesssim
\sum_{j\le j_0}2^j|\Omega|+\delta^{-p}\,\|D^2 v\|^p_{L^p(\Omega)}
\sum_{j>j_0}(2^{-rp/2})^j.
\]
%
Since 
%
\[
\sum_{j\le j_0}2^j\approx 2^{j_0},
\qquad \sum_{j>j_0}(2^{-rp/2})^j\lesssim 2^{-(rp/2)j_0}=2^{-(p-1)j_0}
\]
%
we can write 
%
\[
\#\marked\lesssim\big(\delta^{-1}+\delta^{-p}\delta^{2(p-1)}\big)
\,|\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}\approx \delta^{-1}
\,|\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}.
\]
%
We finally apply Theorem \ref{nv-T:complexity-refine} (complexity of \REFINE) to arrive at 
%
\[
\#\grid-\#\grid_0\lesssim \#\marked\lesssim\delta^{-1}
\,|\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}.
\]
\step{5} It remains to estimate the energy error. We have, upon
termination of \textsf{GREEDY}, that $e_T(v)\le\delta$ for all
$T\in\grid$. Then 
%
\[
|v-I_\grid v|^2_{H^1(\Omega)}=\sum_{T\in\grid} e_T(v) ^2\le\delta^2\,\#\grid.
\]
This concludes the Theorem.
\end{proof}

By relating the threshold value $\delta$ and the number of refinements
$N$, we obtain a result about the convergence rate.
 
\begin{corollary}[convergence rate]\label{nv-C:optimal-mesh}
Let $v\in H^1_0(\Omega)$ satisfy \eqref{nv-weaker-reg}. 
Then for $N>\#\grid_0$ integer there exists $\grid\in\grids$ such that
%
\[
|v-I_\grid v|_{H^1(\Omega)}\lesssim 
|\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}N^{-1/2},\qquad \#\grid-\#\grid_0\lesssim N.
\]
%
\end{corollary}
\begin{proof}
Choose $\delta^2=|\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}N^{-1}$ in 
Theorem \ref{T:greedy}. Then, there exists 
$\grid\in\grids$ such that $\#\grid-\#\grid_0\lesssim N$ and
%
\begin{align*}
|v-I_\grid v|_{H^1(\Omega)}& \lesssim|\Omega|^{1-1/p}\,\|D^2
v\|_{L^p(\Omega)}N^{-1}\big(N+\#\grid_0\big)^{1/2}
\\
& \lesssim |\Omega|^{1-1/p}\,\|D^2 v\|_{L^p(\Omega)}N^{-1/2}
\end{align*}
%
because $N>\#\grid_0$. This finishes the Corollary.
\end{proof}
\end{comment}


\begin{remark}[piecewise smoothness]\label{R:pw-smooth}
The global regularity \eqref{nv-weaker-reg} can be weakened to
          \emph{piecewise $W^2_p$ regularity} over the
          initial mesh $\grid_0$, namely $W^2_p(\Omega;\grid_0)$,
          and global $H^1_0(\Omega)$. This is
          because $W^2_p(T)\hookrightarrow C^0(\overline{T})$ for all
          $T\in\grid_0$, whence $I_\grid$ can be taken to be
          the Lagrange interpolation operator.
          \todo[inline]{We could already have here an application of Proposition \ref{P:cont-vs-discont}.}
\end{remark}

\begin{remark}[case $p<1$]\label{R:p<1}
We consider now polynomial degree $n\ge1$. The integrability $p$ 
corresponding to differentiability $n+1$ results from equating
Sobolev numbers:
%
\[
n+1-\frac{d}{p}=\sob(H^1)=1-\frac{d}{2}
\quad\Rightarrow\quad p=\frac{2d}{2n+d}.
\]
%
Depending on $d\ge2$ and $n\ge1$, this may lead to $0<p<1$, in which 
case $W^{n+1}_p(\Omega)$ is to be replaced by the Besov space
$B^{n+1}_{p,p}(\Omega)$ \cite{DeVore:98}. The argument
of Theorem \ref{T:greedy} works provided we replace
\eqref{E:termination} by a modulus of regularity; in fact, $D^{n+1}v$ would
not be locally integrable and so would fail to be a distribution.\todo{AB: I am confused here, there are distributions that are not locally integrable.}
\end{remark}

\begin{remark}[\GREEDY for other norms]\label{R:greedy-non-energy}
Algorithm \GREEDY applies to norms $W^m_q$ for $0\le m \le n+1$ and $1\le q \le \infty$, in accordance with
Remark \ref{R:non-energy-norms}. We will exploit this
flexibility and revisit \GREEDY in Section \ref{S:data-approx} to approximate data.
\end{remark}

\begin{remark}[isotropic vs anisotropic elements]\label{R:anisotropic}
Since geometric singularities are of the form \eqref{E:corner-sing} for $d=2$,
Theorem \ref{T:greedy} shows
that isotropic graded meshes can always deal with such
singularities for $d=2$. Unfortunately, this is no longer the case for $d>2$ and
anisotropic meshes are necessary for optimal meshes.
%
\todo[inline]{This is again an opportunity to say something about a topic will
  not dwell upon later.}
\end{remark}

%-------------------------------------------------------------------------------------
\subsection{\bf Nonconforming Meshes}\label{S:nonconforming-meshes}
%-------------------------------------------------------------------------------------
%
More general subdivisions of $\Omega$ than those in 
\S \ref{S:bisection} are used in practice.
If the elements of $\gridk[0]$ are quadrilaterals for $d=2$, or their
multidimensional variant for $d>2$, then it is natural to allow for improper
or {\it hanging nodes} for the resulting refinements $\grid$ to be
graded; see Figure \ref{nv-F:nonconforming-meshes} (a).
On the other hand, if $\gridk[0]$ is made of triangles for $d=2$,
or simplices for $d>2$, then red refinement without green
completion also gives rise to graded meshes with hanging nodes;
see Figure \ref{nv-F:nonconforming-meshes} (b). In both cases, the
presence of hanging nodes is inevitable to enforce mesh grading.
Finally, bisection may produce meshes with hanging nodes, as depicted
in Figure \ref{nv-F:nonconforming-meshes} (c), if the completion
process is incomplete. All three refinements maintain shape
regularity, but for both practice and theory, they
cannot be arbitrary: we need to restrict the level of nonconformity.
We discuss this next.
%
\todo[inline]{I propose to introduce here the notion of global index.
Claudio and I can discuss this matter and make a suggestion. AB: I would suggest to make sure first that this notion extends to 3d. I think it does.}
%
\begin{figure}[ht]
\includegraphics[width=0.27\textwidth]{figs/bisection/quadrilateral_inf}
\hskip0.3cm
\includegraphics[width=0.32\textwidth]{figs/bisection/red_inf}
\hskip0.2cm
\includegraphics[width=0.32\textwidth]{figs/bisection/bisection_inf}
\caption{Nonconforming meshes made of quadrilaterals (a), triangles with 
red refinement (b), and triangles with bisection (c). The shaded
regions depict the domain of influence of a proper or conforming node $P$.}
\label{nv-F:nonconforming-meshes}
\end{figure}

We start with the notion of domain of influence of a proper node,
introduced by Babu\v ska and Miller in the context of $K$-meshes
\cite{BabuskaMiller:87}; see Figure \ref{nv-F:nonconforming-meshes}.
For simplicity, we restrict ourselves to polynomial degree $n=1$.
We say that a node $P$ of $\grid$ is a {\it proper} (or conforming) node if
it is a vertex of all elements containing $P$; otherwise, we say that
$P$ is an {\it improper} (nonconforming or hanging) node. 
Since we only prescribe
degrees of freedom at the proper nodes, it is natural to describe
the canonical continuous piecewise linear basis functions $\phi_P$
associated with each proper node $P$.

We do this recursively. As in \S \ref{S:bisection},
the {\it generation} $g(T)$ of an element $T\in\grid$
is the number of subdivisions needed to create $T$ from its ancestor
in the initial mesh $\gridk[0]$, hereafter assumed to be conforming. 
We first rearrange the elements in
$\grid = \{T_i\}_{i=1}^{\#\grid}$ by generation: $g(T_i)\le
g(T_{i+1})$ for all $i\ge0$.
Suppose that $\phi_P$ has been already defined for each $T\in\grid$
with $g(T)<i$. We proceed as follows to define $\phi_P$ at each vertex
$z$ of $T\in\grid$ with $g(T)=i$:
%
\begin{itemize}
\item
if $z$ is a proper node, then we set $\phi_P(z)=1$ if $z=P$ and
$\phi_P(z)=0$ otherwise;

\item
if $z$ is a hanging node, then $z$ belongs to an edge of another
element $T'\in\grid$ with $g(T')<i$ and set $\phi_P(z)|_T=\phi_P(z)|_{T'}$.
\end{itemize}
%
This definition is independent of the choice of $T'$ since, by
construction, $\phi_P$ is continuous across interelements of lower
level. We also observe that $\{\phi_P\}_{P\in\nodes}$ is a basis of the finite
element space $\V(\grid)$ of {\it continuous} piecewise linear
functions, thus
%
\[
V = \sum_{P\in\nodes} V(P) \phi_P \qquad\forall ~V\in\V(\grid).
\]
%
The {\it domain of influence} of a proper node $P$ is the support of
$\phi_P$:
%
\[
\omega_\grid(T) = \supp (\phi_P).
\]
%
We say that a sequence of nonconforming meshes $\{\grid\}$ is 
{\it admissible} if there is a
universal constant $\Lambda_* \le 1$, independent of the refinement
level and $\grid$, such that 
%
\begin{equation}\label{nv-level-nonconformity}
\diam(\omega_\grid(T)) \le \Lambda_* h_T \qquad\forall ~T\in\grid.
\end{equation}
%
An important example is quadrilaterals with {\it one} hanging node per
edge. We observe, however, that \eqref{nv-level-nonconformity} can neither
be guaranteed with more than
one hanging node per edge for quadrilaterals, nor for triangles with
one hanging node per edge (see Problem \ref{nv-E:level-nonconf}).

Given an admissible grid $\grid$, a subset $\marked$ 
of elements marked for refinement, and a desired number $\rho\ge1$ of
subdivisions to be performed in each marked element, the procedure
%
\[
\gridk[*] = \REFINE (\grid,\marked)
\]
%
creates a minimal admissible mesh $\gridk[*]\ge\grid$ such that all
the elements of $\marked$ are subdivided at least $\rho$ times. In order
for $\gridk[*]$ to be admissible, perhaps other elements not in
$\marked$ must be partitioned. Despite the fact that admissibility is a 
constraint on the refinement procedure weaker than conformity,
it cannot avoid the propagation of refinements beyond $\marked$.
The complexity of $\REFINE$ is again an issue which we discuss
in \S \ref{S:proof-complexity-nonconforming}: we show that 
Theorem \ref{nv-T:complexity-refine} extends to this case.

\begin{lemma}[$\REFINE$ for nonconforming meshes]\label{nv-L:nonconforming-meshes}
Let $\gridk[0]$ be an arbitrary conforming partition of $\Omega$, 
except for bisection in which case $\gridk[0]$ satisfies the labeling
\eqref{nv-initial-label} for $d=2$ or its higher dimensional counterpart
\cite{Stevenson:08}. Then the estimate
%
\[
\#\gridk - \#\gridk[0] \le \Lambda_0 \sum_{j=0}^{k-1} \# \markedk[j]
\quad\forall k\ge 1
\]
%
holds with a constant $\Lambda_0$ depending on $\gridk[0], d$ and $\rho$.
\end{lemma}

We conclude by emphasizing that the polynomial interpolation and adaptive
approximation theories of \S\S \ref{S:pol-interp}
and \ref{S:constructive} extend to nonconforming meshes with fixed
level of incompatibility as well.

%-------------------------------------------------------------------------------------
\subsection{\bf Notes}\label{S:notes-1}
%-------------------------------------------------------------------------------------
%
The use of Sobolev numbers is not so common in the finite element
literature, but allows as to write compact error estimates and speak
about nonlinear Sobolev scale. The latter concept is quite natural in
nonlinear approximation theory \cite{DeVore:98}.

The discussion of bisection for $d=2$ follows Binev, Dahmen, and
DeVore \cite{BiDaDeV:04}. Stevenson extended the theory to $d>2$
\cite{Stevenson:08}. We refer to the survey by Nochetto, Siebert and
Veeser \cite{NoSiVe:09} for a rather complete discussion for $d>1$,
and to \S \ref{S:complexity-refine} for a proof of Theorem
\ref{nv-T:complexity-refine} for $d=2$, which easily extends to $d>2$.

The discussion of finite element spaces
\cite{Braess:01,BrennerScott:08,Ciarlet:02} and polynomial
interpolation \cite{BrennerScott:08,DupontScott:80,ScottZhang:90} is
rather classical. In contrast, the material of adaptive approximation
is much less documented. The principle of equidistribution goes back
to Babu\v ska and Rheimboldt \cite{BabuskaRheinboldt:78} and the a
priori design of optimal meshes for corner singularities for $d=2$ is
due to Babu\v ska, Kellogg, and Pitk{\"a}ranta \cite{BaKePi:79}. The
construction of optimal meshes via bisection using thresholding is
extracted from Binev, Dahmen, DeVore, and Petrushev
\cite{BiDaDeVPe:02}.

Finally the discussion of nonconforming meshes follows Bonito and
Nochetto \cite{BonitoNochetto:09}, and continues in \S 
\ref{S:complexity-refine} with the proof of 
Lemma \ref{nv-L:nonconforming-meshes}.

 


==> univariate.tex <==
%-------------------------------------------------------------------------------------
\subsection{Classical vs Adaptive Pointwise Approximation}\label{nv-S:clas-adap}
%-------------------------------------------------------------------------------------
We start with a simple motivation in 1d for the use of adaptive
procedures, due to DeVore \cite{DeVore:98}.
Given $\Omega=(0,1)$, a partition $\gridN=\{x_i\}_{n=0}^N$ of $\Omega$
%
\[
0=x_0 < x_1 <\cdots < x_n < \cdots < x_N = 1
\]
%
and a continuous function $u:\Omega\to\R$, we consider the problem of
{\it interpolating} $u$ by a {\it piecewise constant} function $\uN$ over 
$\gridN$.
To quantify the difference between $u$ and $\uN$ we resort to the
{\it maximum norm} and study two cases depending on the regularity of $u$.

\bigskip\noindent
{\bf Case 1: $W^1_\infty$-Regularity}. 
Suppose that $u$ is Lipschitz in $[0,1]$. We
consider the approximation
%
\[
\uN(x) \definedas u(x_{n-1}) \qquad\text{for all } x_{n-1}\le x<x_n.
\]
%
Since
%
\[
|u(x)-\uN(x) | = |u(x) - u(x_{n-1})| = \Big|\int_{x_{n-1}}^x
u'(t) dt \Big| \le h_n \|u'\|_{L^\infty(x_{n-1},x_n)}
\]
%
we conclude that
%
\begin{equation}\label{nv-orderN}
  \|u - \uN\|_{L^\infty(\Omega)} \leq \frac{1}{N} \|u'\|_{L^\infty(\Omega)},
\end{equation}
%
provided the local mesh-size $h_n$ is about constant 
({\it quasi-uniform} mesh), and so proportional
to $N^{-1}$ (the reciprocal of the number of degrees of freedom). 
Note that the same integrability is used on both
sides of \eqref{nv-orderN}. A
natural question arises: {\it Is it possible to achieve the same 
asymptotic decay rate $N^{-1}$ with weaker regularity demands?}

\bigskip\noindent
{\bf Case 2: $W^1_1$-Regularity}. To answer this question, we suppose
$\|u'\|_{L^1(\Omega)}=1$ and consider the non-decreasing function
%
\[
\phi(x) := \int_0^x |u'(t)| dt
\]
%
which satisfies $\phi(0)=0$ and $\phi(1)=1$. Let $\gridN=\{x_i\}_{n=0}^N$
be the partition given by
%
\[
\int_{x_{n-1}}^{x_n} |u'(t)| dt = \phi(x_n) - \phi(x_{n-1}) = \frac{1}{N}.
\]
%
Then, for $x\in[x_{n-1},x_n]$,
%
\[
|u(x) - u(x_{n-1})| =  \Big|\int_{x_{n-1}}^x u'(t) dt \Big|
\le \int_{x_{n-1}}^x |u'(t)| dt \le \int_{x_{n-1}}^{x_n} |u'(t)| dt
= \frac{1}{N},
\]
%
whence
%
\begin{equation}\label{nv-linf-l1}
\|u-\uN\|_{L^\infty(\Omega)} \leq \frac{1}{N} \|u'\|_{L^1(\Omega)}.
\end{equation}
%
We thus conclude that we could achieve
the same rate of convergence $N^{-1}$ for rougher functions with just
$\|u'\|_{L^1(\Omega)}<\infty$. The following comments are in order for Case 2.

\begin{remark}[equidistribution]
The optimal mesh $\grid_N$ \emph{equidistributes} the max-error. This mesh is
graded instead of uniform but, in contrast to a uniform mesh, such a partition may not be
adequate for another function with the same basic regularity as $u$.
It is instructive to consider the singular function
$u(x)=x^\gamma$ with $\gamma=0.1$ and error tolerance $10^{-2}$
to quantify the above computations: if $N_1$ and $N_2$ are the number
of degrees
of freedom with uniform and graded partitions, we obtain
$N_1/N_2 = 10^{18}$.
\end{remark}

\begin{remark}[nonlinear Approximation]\label{nv-R:approx-theory}
The regularity of $u$ in \eqref{nv-linf-l1} is measured in $W^1_1(\Omega)$ 
instead of $W^1_\infty(\Omega)$ and, consequently,
the fractional $\gamma$ regularity measured in $L^\infty(\Omega)$
increases to one full derivative when expressed in $L^1(\Omega)$.
This exchange of integrability
between left and right-hand side of \eqref{nv-linf-l1}, and gain of
differentiability, is at the
heart of the matter and the very reason why suitably graded meshes achieve
optimal asymptotic error decay for singular functions. By those we
mean functions which are not in the usual linear Sobolev scale, say 
$W^1_\infty(\Omega)$ in this example, but rather in a 
nonlinear scale \cite{DeVore:98}. We will
get back to this issue in \S\ref{S:conv-rates-coercive}.
\end{remark}

